On strategies for selection games related to countable dimension

Two selection games from the literature, $G_c(\mathcal O,\mathcal O)$ and $G_1(\mathcal O_{zd},\mathcal O)$, are known to characterize countable dimension among certain spaces. This paper studies their perfect- and limited-information strategies, and investigates issues related to non-equivalent characterizations of zero-dimensionality for spaces that are not both separable and metrizable. To relate results on zero-dimensional and finite-dimensional spaces, a generalization of Telg\'{a}rsky's proof that the point-open and finite-open games are equivalent is demonstrated.

==> extrastuff.tex <==

\newpage

\section{Stuff to maybe move into the paper above}



\section{Subspace stuff}

Any subset of a zero-dim\(_X\) set is also zero-dim\(_X\).

If Two can win \(\mathsf G_c(\mathcal O,\mathcal O)\), then Two can win on a closed subset.
Suppose \(F \subseteq X\) is closed.
For any open cover \(\mathscr U\) of \(F\), we can expand it to an open cover \(\hat{\mathscr U}\) of \(X\)
in the following way: first, we can fix a function \(\phi\) so that, for any open \(U \subseteq F\), \(\phi(U) \subseteq X\)
is open and \(\phi(U) \cap F = U\). Then \(\hat{\mathscr U} = \{ X \setminus F \} \cup \phi[\mathscr U]\).
Then, when Two plays against these in the game on \(X\), they can produce a cover of \(X\) which is
surely, once restricted to \(F\), a cover of \(F\) following the rules of play.

If Two can win \(\mathsf G_1(\mathcal O_{0\dim},\mathcal O)\), then Two can win on a closed subset.
Suppose \(F \subseteq X\) is closed.
For any open cover \(\mathscr U\) of \(F\), we can expand it to an open cover \(\hat{\mathscr U}\) of \(X\)
in the following way: first, we can fix a function \(\phi\) so that, for any open \(U \subseteq F\), \(\phi(U) \subseteq X\)
is open and \(\phi(U) \cap F = U\). Then \(\hat{\mathscr U} = \{ \phi(U) \cup (X \setminus F) : U \in \mathscr U\}\).
Then, when Two plays against these in the game on \(X\), they can produce a cover of \(X\) which is
surely, once restricted to \(F\), a cover of \(F\) following the rules of play.


Using a bijection \(\omega^2 \to \omega\), it should be the case that we can extend these to \(F_\sigma\) subsets.
That is, if Two can win on \(X\), then Two can also win on the restriction of the game to any \(F_\sigma\) subset of \(X\).
.....


Don't forget the equivalence of finite open covers....
In fact, for any paracompact space \(X\), \(\dim X = 0\) if and only if ever open cover
consisting of two open sets has an open shrinking which is pairwise disjoint and covers the space.
Can we somehow then restrict player One to only play pairs of open sets that cover the space?

\section{Playing on the Hilbert Cube}

What if we just play on \([0,1]^\omega\) and see what subsets One has a winning strategy on?
If we can show those sets are the same, perhaps this establishes equivalence of the games for
separable metrizable spaces, at least.
As we know, Two can win either game only on countable-dimensional subspaces of \([0,1]^\omega\).
We also know how to translate winning strategies for One in \(\textsf{G}_c(\mathcal O,\mathcal O)\) to
winning strategies for One in \(\textsf{G}_1(\mathcal O_{0\dim},\mathcal O)\).
To do this, consider any open cover \(\mathscr U\) of \([0,1]^\omega\).
For every zero-dimensional \(Z\), let \(\mathscr V_Z\) be a pairwise disjoint refinement of \(\mathscr U\)
that covers \(Z\).
Then One plays \(\{ \bigcup \mathscr V_Z : Z \text{ is zero-dim}\}\) in the other game.
Whatever Two picks corresponds to \emph{some} pairwise disjoint refinement of \(\mathscr U\)
and we can pick one of them.
Now, since One was playing according to some winning strategy, we see that Two did not cover the target space
in either game.


So now the question is, if One can win \(\textsf{G}_1(\mathcal O_{0\dim},\mathcal O)\)
relative to \(X \subseteq [0,1]^\omega\), can One also win \(\textsf{G}_c(\mathcal O,\mathcal O)\) there?
Somehow we need to relate One's responses to just one open set...
We can probably let One open up with the exact same open cover they would use in
\(\textsf{G}_1(\mathcal O_{0\dim},\mathcal O)\).
However, in \(\textsf{G}_c(\mathcal O,\mathcal O)\), Two gets to pick a countable family of pairwise
disjoint open sets, say \(\mathscr V\) that refines \(\mathscr U\).
The problem is that \(\bigcup \mathscr V\) might not be an element of \(\mathscr U\).
Can we get an element of \(U\) that is \emph{close enough}?
One thing to note is that, for any countable \(E \subseteq \bigcup \mathscr V\),
there is some \(U \in \mathscr U\) so that \(E \subseteq U\).
So we can find \(U \in \mathscr U\) that are \emph{dense} in \(\bigcup \mathscr V\).
What would be super duper cool is if we could get \(U\in\mathscr U\) so that
\(\bigcup \mathscr V \subseteq U\).

Note: Since the Hilbert cube isn't a \(C\)-space, One has a predetermined winning strategy
in the Haver game.

Undetermined sets???


Notice that there are \(\mathfrak c\) many \(G_{\delta\sigma}\) countable-dimensional
subsets of the Hilbert cube.
If we assume CH, then we can enumerate them: \(\{ E_\alpha : \alpha < \omega_1 \}\).
Then, for each \(\alpha < \omega_1\) let \(x_\alpha \not\in \bigcup_{\beta \leq \alpha} E_\beta\).
Observe that \(\{ x_\alpha : \alpha < \omega_1 \}\) is not countable-dimensional.
If it were, it could be written as the countable union of zero-dimensional subsets
which are all contained in \(G_\delta\) zero-dimensional subsets, but then the union
of these \(G_\delta\) subsets is a \(G_{\delta\sigma}\) countable-dimensional subset.
That is, Two has no winning strategy for this set.
\textcolor{red}{Verify this claim. Check for separability.}
\textcolor{black!30!green}{Separability is true since we are working with a subspace of a separable metric space.}
So what about One?


\(\mathsf S_1(\mathcal O_{0\dim},\mathcal O) \implies \mathsf S_c(\mathcal O,\mathcal O)\):
Let \(\mathscr U_n\) be an open cover of \(X\) and define
\[\mathscr V_n = \left\{ \bigcup \mathscr W : \mathscr W \text{ is a pairwise disjoint refinement of }\mathscr U \right\}.\]
We can apply \(\mathsf S_1(\mathcal O_{0\dim},\mathcal O)\) to pick out \(V_n \in \mathscr V_n\) so that
\(X = \bigcup_n V_n\) and each \(V_n\) corresponds to a pairwise disjoint refinement of \(\mathscr U_n\) so we're done.



Suppose \(\mathsf S_1(\mathcal O_{0\dim},\mathcal O)\) fails and let \(\mathscr U_n\) be the witnessing sequence
of this failure.
Since we are considering a separable metric space, each collection of pairwise disjoint refinements is at most countable.
Consider \(\mathscr V_n\) a pairwise disjoint refinement of \(\mathscr U_n\).
For any countable dense subset \(D\) of \(\bigcup \mathscr V_n\), there exists \(U_n \in \mathscr U_n\) so that \(D \subseteq U_n\).
Notice that the \(U_n\) cannot cover \(X\)....
In fact, for any \(\varphi : \omega \to \bigcup_n \mathscr U_n\) so that \(\varphi(n) \in \mathscr U_n\),
\[F_\varphi := X \setminus \bigcup_n \varphi(n) \neq \emptyset.\]

Notice that if One has a winning strategy in \(\mathsf G_c(\mathcal O,\mathcal O)\), then One has a winning strategy
in the Rothberger game, \(\mathsf G_1(\mathcal O,\mathcal O)\).
Indeed, One need only play the same strategy since Two's single selection is also a collection of pairwise
disjoint open sets.
Now, see \cite{zbMATH00695594} for the implication that there
exists some closed set \(F \subseteq X \times \omega^\omega\) so that each \(F_x = \{ y \in \omega^\omega : \langle x, y \rangle \in F \}\)
is nowhere dense in \(\omega^\omega\) and \(\omega^\omega = \bigcup_{x \in X} F_x\).
Is there a similar approach here?
Maybe we can get an equivalent condition with a closed nowehere dense \(F\)...
That doesn't seem quite right since the definition of the set is very much based on the Rothberger game.
Effectively, Rec{\l}aw is using \(\omega^\omega\) to code Two's possible responses seen as a single selection
from a set of integers.

If One has a winning strategy in \(\mathsf G_c(\mathcal O,\mathcal O)\), can we produce something similar?
Note that One can win using basic open covers.
So fix a countable basis \(\mathcal B = \{ B_n : n \in \omega \}\).
Player One is effectively choosing a finite (by compactness) subset of \(\mathcal B\).
Player Two however is effectively picking a countable subset of \(\omega\).
So that doesn't seem particularly promising.



How about this instead?
One is still picking a finite subset of \(\mathcal B\), but Two is just playing the
complement of the union of their selection.
I guess we should determine if One's strategy can just respond to the union of Two's plays instead of the cover itself.

\begin{proposition}
    If One has a winning strategy in \(\mathsf G_c(\mathcal O,\mathcal O)\),
    One has a winning strategy which only responds to the union of Two's responses in each inning.
\end{proposition}
\begin{proof}
    Suppose One has a winning strategy in \(\mathsf G_c(\mathcal O,\mathcal O)\).
    For any open cover \(\mathscr U\), define \(\mathrm{pdr}(\mathscr U)\) to be the set of all pairwise
    disjoint refinements of \(\mathscr U\).
    Define a relation \(\sim\) so that, for \(\mathscr V , \mathscr W \in \mathrm{pdr}(\mathscr U)\), \(\mathscr V \sim \mathscr W\)
    iff \(\bigcup \mathscr V = \bigcup \mathscr W\).
    Define a choice \[\gamma_{\mathscr U} : \{ [\mathscr V]_\sim : \mathscr V \in \mathrm{pdr}(\mathscr U) \} \to \mathrm{pdr}(\mathscr U)\]
    so that \(\gamma_{\mathscr U}([\mathscr V]_\sim) \in [\mathscr V]_\sim\).
    Then we can adjust One's strategy to play uniformly on these equivalence classes.
    Namely, if One plays \(\mathscr U\) and Two chooses \(\mathscr V \in \mathrm{pdr}(\mathscr U)\), then
    One pretends that Two has played \(\gamma_{\mathscr U}([\mathscr V]_\sim)\).
    
    Now, let's see that this modified strategy is still winning.
    The opening play has not changed; that is, One opens with some \(\mathscr U_0\).
    Given a response \(\mathscr V_0 \in \mathrm{pdr}(\mathscr U_0)\), One responds
    with \(\mathscr U_1\) according to \(\gamma_{\mathscr U_0}([\mathscr V_0]_\sim)\).
    We can continue in this way.
    Since the game played according to Two's responses with \(\mathscr W_n := \gamma_{\mathscr U_n}([\mathscr V_n]_\sim)\)
    are according to the winning strategy, \(\bigcup_n \bigcup \mathscr W_n\) cannot cover the space.
    Since \(\bigcup \mathscr W_n = \bigcup \mathscr V_n\) for each \(n\), we see that the modified strategy is also winning.
\end{proof}



For any open cover \(\mathscr U\), let \(\mathscr U^\ast = \left\{ \bigcup \mathscr V : \mathscr V \in \mathrm{pdr}(\mathscr U) \right\}\).
Now, it should be the case that \(\mathscr U^{\ast\ast} = \mathscr U^\ast\).
Let \(\mathscr W \in \mathrm{pdr}(\mathscr U^\ast).\)
For each \(W \in \mathscr W\), let \(\mathscr V(W) \in \mathrm{pdr}(\mathscr U)\) be so that
\(W \subseteq \bigcup \mathscr V(W)\).
Then we can consider \(\mathscr W_W = \{ V \cap W : V \in \mathscr V(W) \}\).
Notice that \(\mathscr W_W\) is pairwise disjoint and refines \(\mathscr U\).
Since \(\mathscr W\) was pairwise disjoint, we see that the family \(\bigcup \{ \mathscr W_W : W \in \mathscr W \}\)
is a pairwise disjoint refinement of \(\mathscr U\).
Also, \(\bigcup \bigcup \{ \mathscr W_W : W \in \mathscr W \} = \bigcup \mathscr W\).

So I think the question is this: If One has a winning strategy with zero-dim covers and Two gets to make a single selection,
can One still win where we apply this operation to the covers in their strategy?
In some sense, the question is: how close are zero-dim covers to being closed under unions?


So this is starting to sound like the following single selection game:
One plays a set \(\mathcal F_n\) of closed subsets, and Two selects one closed subset \(F_n \in \mathcal F_n\).
Two wins if \(\bigcap_n F_n = \emptyset\).
However, as commented elsewhere, these probably aren't equivalent.
The potential problem is that some set \(\mathcal F_n\) of closed sets probably doesn't necessarily correspond
to some unique open cover \(\mathscr U\) of the space.
In particular, as we show below, one necessary condition for that is for \(\mathcal F_n\) to be closed
under superset.

\section{Random hyperspace dreaming}

In the \(\mathsf G_c(\mathcal O, \mathcal O)\) game, One plays open covers and Two, without loss of generality, can play
a pairwise disjoint refinement where the union is dense.
Now, for a given open cover, there is a corresponding set of closed nowhere dense sets that result as a complement of a pairwise
disjoint dense refinement of that open cover.
So what if instead we look at the following game on the space of closed nowhere dense sets:
Player One will choose a collection of closed nowhere dense sets and Two gets to pick a particular set from this collection.
Could this get us anything?
Could it be the case that, given a fixed open cover, the resulting complements of pairwise disjoint
dense refinements is open in the Vietoris topology?
What I do suspect is that we will lose too much information in this modification.
What is mean is the following.
Let \(\mathcal M\) denote the space of closed nowhere dense subsets of a compact metrizable space \(X\).
Then we define \(\varphi : \mathcal O_X \to \wp(\mathcal M)\) by the rule
\[
    \varphi(\mathscr U) = \left\{ X \setminus \left( \bigcup \mathscr V \right) : \mathscr V
    \text{ is a pairwise disjoint dense refinement of } \mathscr U\right\}.
\]
This function is probably not onto.

Let \(\mathbb K(X)\) be the set of non-empty compact subsets of \(X\) with the Vietoris topology;
that is, the topology with subbasic elements of the form \(\{ K \in \mathbb K(X) : K \subseteq U \}\)
and \(\{ K \in \mathbb K(X) : K \cap U \neq\emptyset \}\) for open \(U \subseteq X\).

\begin{proposition}
    If \(X\) is compact metrizable with no isolated points, then \[\{ K \in\mathbb K(X) : K \text{ is nowhere dense} \}\]
    is a dense \(G_\delta\).
    It follows that the set of nowhere dense subsets of a compact metrizable space is Polishable.
\end{proposition}
\begin{proof}
    The map \(\langle K , L \rangle \to K \cup L\), \(\mathbb K(X)^2 \to \mathbb K(X)\), is continuous.
    To see this, we consider subbasic elements.
    If \(K_0 \cup L_0 \subseteq U\), then \(K_0 \subseteq U\) and \(L_0 \subseteq U\).
    Then \(\{ K : K \subseteq U \} \times \{ L : L \subseteq U \}\) is the desired neighborhood.
    
    Now, suppose \((K_0 \cup L_0) \cap U \neq \emptyset\).
    The desired neighborhood should be
    \[
        \left(\{ K : K \cap U \neq\emptyset \} \times \mathbb K(X)\right) \cup \left(\mathbb K(X) \times \{ L : L \cap U \neq\emptyset \} \right).
    \]
    
    Assuming \(X\) is compact, for any open set \(U \subseteq X\), \(X \setminus U\) is compact.
    Suppose \(\emptyset \neq U \subsetneq X\).
    Then \(K \mapsto \langle X \setminus U , K \rangle\), \(\mathbb K(X) \to \mathbb K(X)^2\) is continuous.
    It follows that \(K \mapsto K \cup (X \setminus U)\) is continuous.
    Hence, \(\{ K : K \cup (X \setminus U) = X \}\) is closed.
    Notice that \(K \cup (X \setminus U) = X\) if and only if \(U \subseteq K\).
    That is, \(\{ K : U \subseteq K \}\) is closed.
    
    
    Another way to see this is the following:
    Consider \(\{ K : U \not\subseteq K \}\).
    For \(K_0\) in this set, there exists \(x \in U\) so that \(x \not\in K_0\).
    Since \(x \not\in K_0\), we can find open \(V\) so that \(x \in V\) and \(\text{cl}(V) \cap K_0 = \emptyset\).
    Now we can define \(\{ K : K \cap \text{cl}(V) = \emptyset \}\), a neighborhood of \(K_0\).
    Also notice that, for any \(K\) so that \(\text{cl}(V) \cap K = \emptyset\),
    we have that \(U \not\subseteq K\) since \(x \in U \cap \text{cl}(V)\).
    
    Now, if we have a countable basis \(\{ U_n : n \in \omega \}\) for \(X\),
    a closed set \(K\) has nonempty interior if and only if there is some \(n\)
    so that \(U_n \subseteq K\).
    Hence, \[\{ K : \exists n \in \omega \left( U_n \subseteq K \right) \}\] is an \(F_\sigma\) set.
    It follows that the closed nowhere dense sets forms a \(G_\delta\) subset of \(\mathbb K(X)\).
    One may also note, if we assume \(X\) has no isolated points, that the space of
    closed nowhere dense sets is also dense since it will contain the finite subsets.
\end{proof}

\textsc{Comment:} Noting the following more out of curiosity than anything else.
I doubt it is helpful since it can't capture the \(G_\delta\) zero-dimensional subsets.
\begin{proposition}
    For a compact metrizable space \(X\), the set
    \[
        \{ K \in \mathbb K(X) : K \text{ is zero-dimensional}\}
    \]
    is a dense \(G_\delta\).
\end{proposition}
\begin{proof}
    Density follows immediately from the fact that this set contains the finite subsets.
    
    First, we note that, given an open cover \(\mathscr U\) of \(X\), the set
    \[
        \mathfrak S(\mathscr U) := \left\{ K : \exists \mathscr V \text{ a pairwise disjoint refinement of }\mathscr U \left( K \subseteq \bigcup\mathscr V \right) \right\}
    \]
    is open.
    Let \(\mathscr U_n = \{ B(x,2^{-n}) : x \in X \}\) and notice that \(\bigcap_{n \in \omega} \mathfrak S(\mathscr U_n)\) is a \(G_\delta\).
    To finish the proof, we just need to show that
    \[
        \{ K \in \mathbb K(X) : K \text{ is zero-dimensional}\} = \bigcap_{n \in \omega} \mathfrak S(\mathscr U_n).
    \]
    By compactness, we can use the Lebesgue covering number here to finish it off.
\end{proof}


We maybe want to understand, given an open cover \(\mathscr U\),
\[
    \left\{ X \setminus \bigcup \mathscr V : \mathscr V \in\mathrm{pdr}(\mathscr U) \right\}.
\]
This set seems to be closed under superset.

NOTE: If One has a winning strategy, then none of the above mentioned sets can contain any sets of finite dimension.

\begin{proposition}
    Suppose \(\mathscr U\) and \(\mathscr V\) are two collections of sets.
    Then \[\bigcup \mathscr U \cap \bigcup \mathscr V = \bigcup \left( \mathscr U \wedge \mathscr V \right).\]
\end{proposition}
Hence, given an open cover \(\mathscr U\) of \(X\), the set
\[
    \left\{ K \in \mathbb K(X) : \exists \mathscr V \text{ a pairwise disjoint refinement of }\mathscr U \left( K = X \setminus \bigcup \mathscr V\right) \right\}
\]
is closed under finite unions.

In fact, they seem to be closed under superset.
Let \(K_0 = X \setminus \bigcup \mathscr V\) where \(\mathscr V\) is a pairwise disjoint refinement of \(\mathscr U\)
and suppose \(K_0 \subseteq K \in \mathbb K(X)\).
Then notice that \(\mathscr V' := \{ V \cap (X \setminus K) : V \in \mathscr V\}\) is a pairwise disjoint
refinement of \(\mathscr U\).
Since \(X \setminus K \subseteq X \setminus K_0 = \bigcup \mathscr V\), we have that
\[X \setminus K = (X \setminus K) \cap \bigcup \mathscr V = \bigcup \mathscr V'.\]





\newpage



{\color{red}
\section{Chris overview thoughts}
\begin{itemize}
    \item
    Define \(\mathcal Z_{\text{ind}}(X)\), \(\sigma\mathcal Z_{\text{ind}}(X)\) or \(\mathcal Z^\sigma_{\text{ind}}(X)\), and \(\mathcal Z_{\text{dim}}(X)\), \(\sigma\mathcal Z_{\text{dim}}(X)\) or \(\mathcal Z^\sigma_{\text{dim}}(X)\).
    \item
    cite results for metrizable \(X\) so that \(\text{ind} X = 0\) but \(\dim X = 1\).
    Mention that this example separates the potential results relating to \(\sigma\)-zero dimensionality.
    \item
    Ask whether there is a metrizable space \(X\) so that \(\text{ind} X = 0\) but \(X\) is not \(\sigma\mathcal Z_{\text{dim}}(X)\).
    Maybe it's of the form \(X^\omega\) where \(\text{ind} X = 0\) but \(\dim X = 1\).
    What would be interesting about this particular case is that it would be zero-dimensional in the sense used in the
    Babinkostova-Scheepers paper for one direction but Two would NOT have a winning strategy in either the Haver game or the other game.
    \item
    Though Engelking has \(G_\delta\) enlargement theorem for \(\text{Ind}\) for general metrics, he only states it for \(\text{ind}\) in the \emph{separable} metrizable realm.
    At any rate, \(\text{Ind} = \dim\) for general metrics.
    \item
    We have results for \(\sigma\mathcal Z_{\text{dim}}(X)\) relative to general metric spaces.
    \item
    We also have \(\sigma\mathcal Z_{\text{ind}}(X)\) result at least for separable metric spaces.
    Maybe this can be extended. If not, maybe it's a question.
\end{itemize}
}

\section{Background stuff}

A good reference for basics is \href{https://www.maths.ed.ac.uk/~v1ranick/papers/engelking.pdf}{Engelking's Dimension Theory}.


We have three relevant notions of dimension.

\begin{definition}
    The small inductive dimension \(\text{ind} X\) for a regular space \(X\) is defined as follows:
    \begin{itemize}
        \item
        \(\text{ind} X = -1\) if and only if \(X = \emptyset\)
        \item
        \(\text{ind} X \leq n+1\) if, for every point \(x\in X\) and open \(U\) with \(x \in U\), there exists an open set \(V\) so that \(x \in V \subseteq \text{cl}(V) \subseteq U\) and \(\text{ind} \partial V \leq n\).
        \item
        \(\text{ind} X = n\) if \(\text{ind} X \leq n\) and, for all \(m < n\), \(\text{ind} X \not\leq m\)
    \end{itemize}
\end{definition}

By induction, one can see that \(\text{ind}\) is a topological invariant; i.e. it is preserved under homeomorphism.

Notice that, in particular, \(\text{ind}X = 0\) whenever \(X\) is a non-empty space so that, for every \(x \in X\) and open \(U\) with \(x \in U\), there exists a clopen set \(V\) so that \(x \in V \subseteq U\).

\begin{definition}
    The large inductive dimension \(\text{Ind} X\) for a normal space \(X\) is defined as follows:
    \begin{itemize}
        \item
        \(\text{Ind} X = -1\) if and only if \(X = \emptyset\)
        \item
        \(\text{Ind} X \leq n+1\) if, for every closed set \(F\) and open \(U\) with \(F \subseteq U\), there exists an open set \(V\) so that \(F \subseteq V \subseteq \text{cl}(V) \subseteq U\) and \(\text{Ind} \partial V \leq n\).
        \item
        \(\text{Ind} X = n\) if \(\text{Ind} X \leq n\) and, for all \(m < n\), \(\text{Ind} X \not\leq m\)
    \end{itemize}
\end{definition}

It is immediately clear that \(\text{ind}(X) \leq \text{Ind}(X)\).


\begin{theorem}[Theorem 1.6.5]
    For every normal Lindel{\"{o}}f space \(X\), \(\text{ind}(X) = 0\) iff \(\text{Ind}(X) = 0\).
\end{theorem}


\textcolor{red}{Here, I'll diverge a little from Engelking's definition of covering dimension to make it more sensible in general contexts.}
For a family \(\mathcal A\) of subsets of a set \(X\) that covers \(X\) and \(x \in X\), define \(\text{ord}_x(\mathcal A) = \#\{ A \in \mathcal A: x \in A \}\), where \(\#\) denotes cardinality.
If \(\mathcal A\) is so that \(\text{ord}_x(\mathcal A) < \omega\) for every \(x \in X\), we define \(\text{ord}(\mathcal A) = \sup \{ \text{ord}_x(\mathcal A) - 1 : x \in X \}\).


Recall that \(X\) is paracompact if every open cover of \(X\) admits a locally finitely refinement.
Also note that \(\text{ord}(\mathcal A) = 0\) if and only if \(\mathcal A\) consists of pair-wise disjoint sets.

\begin{definition}
    Let \(X\) be a paracompact space.
    The covering dimension of \(X\) is defined as follows.
    \begin{itemize}
        \item
        \(\text{dim} X \leq n\) if every open cover \(\mathscr U\) of \(X\) admits an open refinement \(\mathscr V\) so that \(\text{ord}(\mathscr V) \leq n\).
        \item
        \(\text{dim} X = n\) if \(\text{dim} X \leq n\) and, for all \(m < n\), \(\text{dim} X \not\leq m\)
    \end{itemize}
\end{definition}

\begin{lemma}
    For a paracompact space \(X\), \(\text{dim}(X) = 0 \implies \text{Ind}(X) = 0\).
\end{lemma}


To get the implication \(\text{Ind}(X) = 0 \implies \text{dim}(X) = 0\), Engelking strongly uses the fact that \(\text{dim}(X) = 0\) if and only if ever \underline{\emph{finite}} open cover admits a pair-wise disjoint open refinement.
We can recover this with some more results since \href{https://mathoverflow.net/questions/228574/two-definitions-of-lebesgue-covering-dimension}{This Math Overflow post} came to the rescue.

\begin{proposition}[Theorem 3.1.4] \label{prop:CoveringDimClosedSubspace}
    Let \(X\) be so that \(\text{dim}(X) = n\) and let \(M \subseteq X\) be closed.
    Then \(\text{dim}(M) \leq n\).
\end{proposition}

\begin{definition}
    Given an open cover \(\mathscr U\) of a space \(X\), we define an open shrinking to be any \(\varphi : \mathscr U \to \mathscr T_X\) so that \(\varphi(U) \subseteq U\) for each \(U \in \mathscr U\) and \(\varphi[\mathscr U]\) covers \(X\).
\end{definition}
\begin{lemma}[Lemma 3.1.9] \label{lemma:LocallyFiniteClosedShrinking}
    Suppose \(X\) has a locally finite closed cover \(\mathscr F\) so that \(\text{dim}(F) \leq n\) for each \(F \in \mathscr F\).
    Also suppose \(\mathscr U\) is an open cover of \(X\) so that, for each \(F \in \mathscr F\), \(\#\{ U \in \mathscr U : U \cap F \neq \emptyset \} < \omega\).
    Then \(\mathscr U\) admits an open shrinking \(\mathscr V\) so that \(\text{ord}(\mathscr V) \leq n\).
\end{lemma}

\begin{theorem}[Dowker's Theorem, Theorem 3.2.1]
    For a paracompact space \(X\), the following are equivalent.
    \begin{enumerate}[label=(\alph*)]
        \item \label{DowkerDim}
        \(\text{dim}(X) \leq n\)
        \item \label{DowkerFiniteA}
        For every finite cover \(\mathscr U\) of \(X\), there exists an open shrinking \(\mathscr V\) of \(\mathscr U\) so that \(\text{ord}(\mathscr V) \leq n\).
        \item \label{DowkerFiniteB}
        For every finite cover \(\mathscr U\) of \(X\), there exists an open refinement \(\mathscr V\) of \(\mathscr U\) so that \(\text{ord}(\mathscr V) \leq n\).
    \end{enumerate}
\end{theorem}

\begin{theorem}[Theorem 1.6.10]
    For a paracompact space \(X\), \(\dim X \leq n\) if and only if every \((n+2)\)-sized open cover \(\{ U_j : j < n+2 \}\) admits an open shrinking \(\{V_j : j < n + 2 \}\) so that \(\bigcap_{j=0}^{n+1} V_j = \emptyset\).
\end{theorem}

\begin{theorem}[Theorem 1.6.11 but adapted for full generality] \label{thm:ParacompactZero}
    For a paracompact space \(X\), \(\dim X = 0\) if and only if \(\text{Ind}X = 0\).
\end{theorem}
\begin{theorem}
    If \(X\) is a paracompact Lindel{\"{o}}f space, then \(\dim X = 0\) if and only if \(\text{ind} X = 0\).
\end{theorem}

\textcolor{purple}{
THIS IS WRONG : Thm 3.1 of Countable Dimensionality,
A Game, and the Haver Property implies that
for metrizable spaces,
\(\dim X=0\) iff \(\mathrm{ind} X=0\).
}




\textcolor{black!30!blue}{
This paper might be relevant: \href{https://www.ams.org/journals/tran/1990-318-02/S0002-9947-1990-0954600-9/S0002-9947-1990-0954600-9.pdf}{Kulesza. Metrizable Spaces where the Inductive Dimensions Disagree.}
Theorem 3.3. claims to construct a metrizable space \(K\) which is zero-dimensional but has large inductive dimension \(1\).
They also claim in the opening that \(\dim = \text{Ind}\) for metrizable spaces.
So this seems like an example of a metrizable space so that \(\text{ind} = 0\) but \(\dim = 1\).
Also, \href{https://www.ams.org/journals/bull/1962-68-06/S0002-9904-1962-10872-6/S0002-9904-1962-10872-6.pdf}{Roy. Failure of Equivalence of Dimension Concepts for Metric Spaces.}
}



\begin{definition}
    For a regular space \(X\), let \(\mathcal Z_{\text{ind}}(X) = \{ A \subseteq X : \text{ind} A = 0 \}\).
    For a paracompact space \(X\), let \(\mathcal Z_{\text{dim}}(X) = \{ A \subseteq X : \dim A = 0 \}\).
\end{definition}
By virtue of Theorem \ref{thm:ParacompactZero}, we can see that, for any paracompact space \(X\), \(\mathcal Z_{\text{dim}}(X) \subseteq \mathcal Z_{\text{ind}}(X)\).
However, by the above notes, there is a metrizable space \(X\) so that \(\text{ind}(X) = 0\) but \(\dim X = 1\).
Hence, the containment \(\mathcal Z_{\text{dim}}(X) \subseteq \mathcal Z_{\text{ind}}(X)\), even in the context of metrizable spaces, is, in general, strict.


\newpage


\begin{definition}
    Hurewicz (see Babinkostova and Scheepers Haver game) defines \(X\) to be \textbf{countable-dimensional} if \(X = \bigcup_n X_n\) where each \(X_n\) is zero-dimensional.
    There is also the notion of strongly countable-dimensional: \(X\) is \textbf{strongly countable-dimensional} if \(X = \bigcup_n X_n\) where each \(X_n\) is closed in \(X\) and each \(X_n\) is finite-dimensional.
\end{definition}


{   \color{red}
\emph{Comment.} In Babinkostova's paper ``Select Screenability Game and Covering Dimension,'' she uses covering dimension zero in one direction of the proof and small inductive dimension in the other direction.
\begin{itemize}
    \item
    Namely, the first direction is: \(X\) is countable dimensional \(\implies\) Two has a winning strategy in \(\textsf{G}_c^\omega(\mathcal O,\mathcal O)\).
    In this direction, she uses the covering dimension definition.
    \item
    The second direction is: Two has a winning strategy in \(\textsf{G}_c^\omega(\mathcal O,\mathcal O)\) \(\implies\) \(X\) is countable dimensional.
    In this direction, she uses the basis consisting of clopen sets definition.
    This is suspect since there exist metrizable spaces \(X\) so that \(\text{ind} X = 0\) but \(\dim X = 1\).
\end{itemize}
}
{\color{black!30!blue}
Babinkostova's approach can be fixed if having the Haver property implies the space is strongly paracompact.
}




Let \(A \subseteq X\) where \(X\) is metric be zero-dimensional in the covering sense.
For \(\mathscr U_0 = \{B(x,1/2) : x \in A \}\), let \(\mathscr V_0\) be a refinement
that covers \(A\) consisting of pair-wise disjoint open sets.
Then, consider \(\mathscr U_{n+1} = \{ B(x,2^{-n}) : x \in A \}\) and select
\(\mathscr V_{n+1}\),
a refinement of \(\mathscr U_{n+1} \wedge \bigwedge_{j \leq n} \mathscr V_j\) covering \(A\)
by pairwise-disjoint open sets.
Note then that \(\mathscr V_n\) is a collection of pairwise disjoint open sets
of diameter no greater than \(2^{-n}\) that covers \(A\). 
Let \(G = \bigcap_{n < \omega} \bigcup \mathscr V_n\supseteq A\); by construction
\(G\) is \(G_\delta\).
Let \(\mathscr U\) be an open cover of \(G\).
\textcolor{red}{We can find a refinement \(\mathscr V\) of \(\mathscr U\) consisting of pair-wise disjoint sets that covers \(A\).
Maybe we can fatten up \(\mathscr V\) to cover \(G\) but still consist of pair-wise disjoint open sets and still be a refinement of \(\mathscr U\).}
{   \color{black!50!green}
By way of contradiction, suppose that any \(f : \mathscr V \to \mathscr T_X\) so that \(V \subseteq f(V)\), \(f[\mathscr V]\) covers \(G\), and \(f[\mathscr V]\) is a refinement of \(\mathscr U\), there exist \(V_1, V_2 \in \mathscr V\) so that \(f(V_1) \cap f(V_2) \neq \emptyset\).
For each \(x \in G\), let \(\delta_n(x) \in (0,2^{-n})\) be so that \(B(x,\delta_n(x)) \subseteq U\) for some \(U \in \mathscr U\).
For \(V \in \mathscr V\), let \[G_{V,n} = \left\{ E \subseteq G : \forall x \in E [B(x,\delta_n(x)) \cap V \neq \emptyset] \wedge \exists U \in \mathscr U\left[V \cup \bigcup_{x \in E} B(x,\delta_n(x)) \subseteq U\right]\right\}\]
}

Let \(\mathscr V_n\) be a covering of the rationals by pairwise-disjoint
intervals of length no greater than \(2^{-n}\).
Let \(G=\bigcap_{n<\omega}\bigcup\mathscr V_n\). Let \(\mathscr U\) cover \(G\).




Let \(U_0 \in \mathscr U\), we can find \(n\) and \(V(U_0) \in \mathscr V_n\) so that \(V_n \subseteq U_0\).
We just need to cover \(G \setminus V(U)\) now, which is an open set relative to \(G\), since \(G \setminus V(U_0) = G \cap \bigcup \{ V: V \in \mathscr V_n \setminus \{V(U)\}\}\).
Then maybe look at \(U_1 \in \mathscr U\) so that \(U_1 \cap (G \setminus V(U_0) \neq \emptyset\).




Since the closed finite-dimensional subsets of a space form an ideal of closed sets (the dimension of a union of closed sets is the max of the dimensions of the subspaces forming the union \textcolor{red}{-oh no. this result appears in Engelking's book in the context of separable metric spaces.... see Theorem 1.5.8-}), previous results involving ideals of closed sets should apply.
In particular, we should have some full characterization in terms of strong countable-dimensionality.



Now, for any space \(X\), we can say that \(A \subseteq X\) is zero-dimensional if, for any \(x \in A\) and \(U \subseteq X\) which is open, there exists \(V \subseteq X\) open so that \(x \in V \subseteq \text{cl}(V) \subseteq U\) and \(V \cap A = \text{cl}(V) \cap A\).
This should mean that \(A\) is required to be regular, but no separation axiom requirements are set on \(X\).


\begin{example}
The ordinals as a subset of the long line of length
\(\omega_1\) are an example of a zero-dimensional
subspace not contained in a \(G_\delta\) zero-dimensional subspace. Let \(U_n\) be an open set
containing the ordinals. For each \(\alpha\) choose \(f_n(\alpha)<\alpha\) such that
\((f_n(\alpha),\alpha]\subseteq U_n\). By the pressing-down lemma there exists a
stationary (in particular, uncountable) subset \(S_n\subseteq\omega_1\) such that
\(f_n(s)=\gamma_n\) for each \(s\in S_n\). Choose \(\gamma\geq\gamma_n\) for all
\(n<\omega\), and then choose \(s_n\in S_n\) such that \(s_n\geq\gamma+1\) for all \(n<\omega\).
Then we have shown that \((\gamma,\gamma+1]\subseteq(\gamma_n,s_n]=(f_n(s_n),s_n]\subseteq U_n\)
for all \(n<\omega\), so \(\bigcap_{n<\omega} U_n\) always contains a non-zero-dimensional
subset.
\end{example}
\textcolor{red}{Question. Do the ordinals in this example have the property that every open cover admits a pair-wise disjoint refinement that covers the ordinals? It has a relatively clopen basis by looking at \((\beta + 1/2 , \alpha + 1/n)\) where \(\beta < \alpha\).}


\begin{theorem}[Engelking]
Suppose \(X\) is regular and second-countable and \(A \subseteq X\) is zero-dimensional.
We claim that there exists a countable basis \(\mathscr B\) for the topology on \(X\) so that, for each \(B \in \mathscr B\), \(\partial B \cap A = \emptyset\). (Therefore \(A\) is contained
in the \(G_\delta\) set \(X\setminus\bigcup_{B\in\mathscr B}\partial B\).)
\end{theorem}

\begin{proof}
Let \(\mathscr B_0\) be a countable basis for \(X\) and let \(\mathscr B_1 = \{ B \in \mathscr B_0 : B \cap \text{cl}(A) = \emptyset \}\) and \(\mathscr B_2 = \{ B \in \mathscr B_0 : B \cap \text{cl}(A) \neq\emptyset\}\).

Fix \(B \in \mathscr B_1\).
For \(x \in B\), since \(X\) is regular, we can find \(U_{x,B} \subseteq X\) open so that \(x \in U_{x,B} \subseteq \text{cl}(U_{x,B}) \subseteq B\).
Now, let \(V_{x,B} \in \mathscr B_0\) be so that \(x \in V_{x,B} \subseteq U_{x,B}\).
Since \(V_{x,B} \subseteq U_{x,B} \subseteq B \subseteq X \setminus \text{cl}(A)\), we see that \(V_{x,B} \in \mathscr B_1\).
Observe that \(\mathscr V_B = \{ V_{x,B} : x \in B \}\) is a countable set, as it is a subset of \(\mathscr B_1\).
For each \(E \in \mathscr V_B\), let \(W_E \subseteq X\) be open so that \(E \subseteq W_E \subseteq \text{cl}(W_E) \subseteq B\) and then \(\mathscr W_B = \{ W_E : E \in \mathscr V_B\}\).
Moreover, since \(B \subseteq X \setminus \text{cl}(A)\), notice that \(\partial W \cap A = \emptyset\) for each \(W \in \mathscr W_B\).

Now fix \(B \in \mathscr B_2\).
For any \(x \in A \cap B\), let \(U_{x,B} \subseteq X\) be open so that \(x \in U_{x,B} \subseteq \text{cl}(U_{x,B}) \subseteq B\) and \(U_{x,B} \cap A = \text{cl}(U_{x,B}) \cap A\).
Now, let \(V_{x,B} \in \mathscr B_0\) be so that \(x \in V_{x,B} \subseteq U_{x,B}\).
Since \(x \in V_{x,B} \cap A\), we see that \(V_{x,B} \in \mathscr B_2\).
Observe that \(\mathscr V_B = \{ V_{x,B} : x \in B \}\) is a countable set as it is a subset of \(\mathscr B_2\).
For each \(E \in \mathscr V_B\), pick \(W_E\) open so that \(E \subseteq W_E \subseteq \text{cl}(W_E) \subseteq B\) and \(W_E \cap A = \text{cl}(W_E) \cap A\).
Define \(\mathscr W_B = \{ W_E : E \in \mathscr V_B \}\).
Notice that, by construction, \(\partial W \cap A = \emptyset\) for each \(W \in \mathscr W_B\).

We now define
\[
    \mathscr B = \bigcup \{ \mathscr W_B : B \in \mathscr B_0 \}.
\]
As a countable union of countable sets, \(\mathscr B\) is countable.
Notice that \(\partial B \cap A = \emptyset\) for all \(B \in \mathscr B\).
So the only thing to show is that \(\mathscr B\) is a basis for \(X\).
We proceed by cases.

Suppose \(x \not\in \text{cl}(A)\) and let \(U\) be open so that \(x \in U \subseteq X \setminus \text{cl}(A)\).
Then we can find \(B \in \mathscr B_0\) so that \(x \in B \subseteq U\).
Clearly, \(B \in \mathscr B_1\).
There is some \(V \in \mathscr V_B\) so that \(x \in V \subseteq B\).
Observe that \(W_V\) is so that \(V \subseteq W_V \subseteq B\subseteq U\).
Hence, \(W_V \in \mathscr B\) is so that \(x \in W_V \subseteq U\).

Suppose \(x \in \text{cl}(A)\) and let \(U\) be open so that \(x \in U\).
Then there is some \(B \in \mathscr B_0\) so that \(x \in B \subseteq U\).
Clearly, \(B \in \mathscr B_2\).
\textcolor{red}{It seems like we'll have to resort to separability to finish this off.... That's okay since second-countable implies separable. Engelking also uses that closed sets are \(G_\delta\), which is true in the context of metric spaces.
See Theorem 1.2.14.
Maybe this argument can be generalized to use weight and density, but then so what?}
\end{proof}

Anyway, for separable metric spaces, every zero-dimensional subset is contained in a zero-dimensional \(G_\delta\).
Are there more spaces where this is true?
Namely, what can we say about \(X\) if every zero-dimensional subset is contained in a zero-dimensional \(G_\delta\)?


{\color{purple}
\begin{theorem}\label{metgdeltazd}
Let \(X\) be metrizable. Then every \(\dim X=0\)
subspace of \(X\) is contained in a \(G_\delta\)
\(\mathrm{ind} X=0\) subspace.
\end{theorem}
\begin{proof}
Let \(A\subseteq X\) satisify
\(\mathrm{dim} A=0\), so we may construct open
covers \(\mathcal U_n\) of \(A\)
such that \(\mathcal U_{n+1}\)
refines \(\mathcal U_n\), \(\mathcal U_n\) is
pairwise disjoint, and each set in \(\mathcal U_n\)
has diameter \(\leq 1/2^n\).

Consider \(B=\bigcap_{n<\omega}\bigcup\mathcal U_n\supseteq A\).
By construction, \(B\) is \(G_\delta\). Let \(x\in B\)
and \(\epsilon>0\). Choose \(n<\omega\) with
\(1/2^n<\epsilon\), and then choose
\(U\in\mathcal U_n\) such that \(x\in U\) and
\(\mathrm{diam} U\leq 1/2^n<\epsilon\). It follows
that \(U\cap B\) is open in \(B\),
and its complement in \(B\), that is to say
\(\bigcup(\mathcal U_n\setminus\{U\})\cap B\), is open
in \(B\). Therefore each point of \(B\) has a basis
of sets clopen in \(B\), showing \(\mathrm{ind} B=0\).
\end{proof}

\begin{corollary}
Let \(X\) be strongly paracompact metrizable. Then every
zero-dimensional subspace is contained in a \(G_\delta\)
zero-dimensional subspace.
\end{corollary}
}

{\color{black!30!blue}
The papers linked above show that a metrizable space \(X\) exists so that \(\text{ind} X = 0\) but \(\dim X = 1\).
This might not be a problem if \(\text{ind} X = 0\) always implies \(\dim X\) is actually finite... However, that
may also not be true.}

%=============================================================================================
%   KURATOWSKI BEGIN    ======================================================================
%=============================================================================================


\newpage
\section{Kuratowski Things}


\textcolor{red}{\emph{Comment.} I've included the following notes I had prepared for myself earlier this summer
when starting to look at Babinkostova's papers on dimension. In particular, Theorem \ref{theorem:EnGdelta}
might be useful to us. Babinkostova refers to Theorem \ref{theorem:FinitePairwiseDisjointSubsace} to construct
coherent plays for Two in the \(\mathsf{G}_c(\mathcal O,\mathcal O)\) game.}


Kuratowski defines the dimension of a space in the following way.
\textcolor{red}{Note! This is Kuratowski's notation but not the covering dimension. It lines up with the small inductive dimension.}
\begin{definition}
	For a regular space \(X\),
	\begin{itemize}
		\item
		\(\dim X = -1\) if and only if \(X = \emptyset\).
		\item
		and a point \(x\in X\), \(\dim_x X \leq n + 1\) if there exists a basis \(\mathcal N\) at \(x\) so that, for all \(U \in \mathcal N\), \(\dim \partial U \leq n\).
		\item
		and a point \(x \in X\), \(\dim_x X = n\) if \(\dim_x X \leq n\) and, for all \(m < n\), \(\dim_x X \not\leq m\).
		\item
		\(\dim X = \sup \{ \dim_x X : x \in X \}\).
	\end{itemize}
\end{definition}
Recall that, for an open set \(U\),
\[\partial U = \overline{U} \cap \overline{X \setminus U} = \overline{U} \cap (X \setminus U) = \overline{U} \setminus U.\]

\begin{theorem}[Monotonicity of Dimension] \label{theorem:Monotonicity}
Suppose \(E \subseteq X\). Then \(\dim E \leq \dim X\).
\end{theorem}
\begin{proof}
	The claim holds true for dimension \(-1\).
	Suppose it holds up to \(n\) and assume \(\dim X = n+1\).
	Let \(p \in E\) and let \(\mathcal N\) be a basis at \(p\) consisting of \(U\) so that \(\dim \partial U \leq n\).
	First, observe that \(\{ U \cap E : U \in \mathcal N \}\) is a basis at \(p\) in \(E\).
	Then,
	\begin{align*}
		\partial_E (U \cap E)
		&= \text{cl}_E(U \cap E) \cap \text{cl}_E(E \setminus U)\\
		&= E \cap \overline{U \cap E} \cap \overline{E \setminus U}\\
		&\subseteq \overline{U} \setminus U\\
		&= \partial U
	\end{align*}
	which, by induction, means that \(\dim \partial_E (U \cap E) \leq \dim \partial U \leq n\).
	Since this holds for arbitrary \(p \in E\), we see that \(\dim E \leq \dim X\).
\end{proof}
\begin{definition}
	Two sets \(A\) and \(B\) are said to be \emph{separated} if \(A \cap \overline{B} = \overline{A} \cap B = \emptyset\).
\end{definition}
\begin{lemma}\label{lem:BoundarySeparation}
	In a hereditarily normal space \(X\), if \(A\) and \(B\) are separated, then there exists an open set \(U\) so that \(A \subseteq U\) and \(\overline{U} \cap B = \emptyset\).
	Moreover, for any open set \(W\) so that \(A \subseteq W \subseteq U\), we also have that \(\overline{W} \cap B = \emptyset\).
\end{lemma}
\begin{proof}
	Consider \(E = X \setminus \left( \overline{A} \cap \overline{B} \right)\).
	Now consider the sets \(A^\ast = \overline{A} \setminus \overline{B}\) and \(B^\ast = \overline{B} \setminus \overline{A}\).
	Notice that \(A^\ast \cap B^\ast = \emptyset\), that
	\[\overline{A} \cap E = \overline{A} \setminus \left(\overline{A} \cap \overline{B}\right) = A^\ast,\]
	and that, similarly, \(\overline{B} \cap E = B^\ast\).
	That is, \(A^\ast\) and \(B^\ast\) are disjoint closed sets in \(E\).
	So we can find disjoint open sets \(U\) and \(V\) relative to \(E\) so that \(A^\ast \subseteq U\) and \(B^\ast \subseteq V\).
	As \(E\) is open in \(X\), \(U\) is also open in \(X\).

	Observe that \[A = A \setminus \overline{B} \subseteq \overline{A} \setminus \overline{B} = A^\ast \subseteq U.\]

	For any open \(W\) so that \(A \subseteq W \subseteq U\), observe that \(\overline{W} \subseteq \overline{U}\).
	Also, as \(U \cap V = \emptyset\), \(W \cap V = \emptyset\) and \(W \subseteq X \setminus V\) which further provides
	\[\overline{W} \subseteq X \setminus V \subseteq X \setminus B^\ast
	= X \setminus (\overline{B} \setminus \overline{A})
	= \left(X \setminus \overline{B}\right) \cup \overline{A}.\]
	Hence,
	\[
		\overline{W} \cap B \subseteq \left( \left(X \setminus \overline{B}\right) \cup \overline{A} \right) \cap B = \emptyset.
	\]
\end{proof}
\begin{theorem} \label{theorem:SubspaceDimension}
	Let \(X\) be a metric space with metric \(d\).
	For a point \(p \in E\) where \(E \subseteq X\), \(\dim_p E \leq n+1\) if and only if there exists a basis \(\mathcal N\) at \(p\) in \(X\) so that, for all \(U \in \mathcal N\), \(\dim( E \cap \partial U ) \leq n\).
\end{theorem}
\begin{proof}
	Suppose such a basis \(\mathcal N\) exists.
	Then notice that \(\partial_E (U \cap E) \subseteq E \cap \partial U\) and that \(\{ U \cap E : U \in \mathcal N \}\) is a basis at \(p\).
	By the monotonicity of dimension, \(\dim \partial_E (U \cap E) \leq \dim \partial U \leq n\).

	On the other hand, suppose \(\dim_p(E) \leq n+1\) and let \(\mathcal V\) be a basis at \(p\) relative to \(E\) so that, for all \(V \in \mathcal V\), \(\partial_E V \leq n\).
	Notice that \(V\) and \(E \setminus \overline{V}\) are separated, so, by Lemma \ref{lem:BoundarySeparation}, we can find open \(W \subseteq X\) so that \(V \subseteq W\) and \(\overline{W} \cap \left(E \setminus \overline{V}\right) = \emptyset\).
	Now, let \(\delta > 0\) be arbitrary and, for each \(v \in V\), let \(r_v > 0\) be so that \(2r_v < \delta\) and \(B(v,r_v) \subseteq W\).
	Let \(U_{V,\delta} = \bigcup\{B(v,r_v):v\in V\}\) and notice that \(U_{V,\delta}\) is open with the properties that \(V \subseteq U_{V,\delta} \subseteq W\) and \(\overline{U}_{V,\delta} \cap \left( E \setminus \overline{V} \right) = \emptyset\) by Lemma \ref{lem:BoundarySeparation}.
	Hence \(X \setminus U_{V,\delta} \subseteq X\setminus V\) and \(E \cap \overline{U}_{V,\delta} \subseteq \overline{V}\) which provides
	\[
		E \cap \partial U_{V,\delta} = E \cap \left(\overline{U}_{V,\delta} \setminus U_{V,\delta}\right) \subseteq E \cap \left( \overline{V} \setminus V \right) = \partial_E V.
	\]
	So, by monotonicity of dimension, \(\dim(E \cap \partial U_{V,\varepsilon}) \leq \dim \partial_E V \leq n\).

	The last thing to see is that \(\mathcal N := \{ U_{V,\delta} : V \in \mathcal V, \delta > 0\}\) forms a basis at \(p\).
	Consider \(B(p,\varepsilon)\) for arbitrary \(\varepsilon > 0\), let \(\delta = \varepsilon/2\), and let \(V \in \mathcal V\) be so that \[V \subseteq B(p,\delta) \subseteq B(p,2\delta) \subseteq B(p,\varepsilon).\]
	By construction,
	\[
		U_{V,\delta} \subseteq \bigcup \{ B(v,\delta/2) : v \in V \}.
	\]
	Let \(y \in U_{V,\delta}\) and let \(v \in V\) be so that \(d(v,y) < r_v < \delta/2\).
	Observe that
	\[
		d(y,p) \leq d(y,v) + d(v,p) < \frac{\delta}{2} + \delta = \frac{3\delta}{2} < 2\delta = \varepsilon.
	\]
	That is, \(U_{V,\delta} \subseteq B(p,\varepsilon)\) which establishes that \(\mathcal N\) is a basis at \(p\).
\end{proof}

\begin{definition}
	Let \(X\) be a metric space and fix \(E \subseteq X\).
	We define \[E_{(n)} = \{ p \in X : \dim_p(E \cup \{p\}) \leq n \}.\]
\end{definition}
Note that, by Theorem \ref{theorem:SubspaceDimension}, \(p \in E_{(n)}\) if and only if there exists a basis \(\mathcal N\) at \(p\) consisting of sets \(U\) so that \(\dim(E \cap \partial U) < n\).
\begin{proposition}
	For any \(E \subseteq X\) where \(X\) is a metric space, \(\dim(E \cap E_{(n)}) \leq n\).
\end{proposition}
\begin{theorem} \label{theorem:EnGdelta}
	For a metric space \(X\) with metric \(d\) and \(E \subseteq X\), \(E_{(n)}\) is a \(G_\delta\) set.
\end{theorem}
\begin{proof}
	For each \(x \in E_{(n)}\), let \(U_{x,k}\) be a neighborhood of \(x\) so that \(U_{x,k} \subseteq B(x,2^{-k})\) and \(\dim(E \cap \partial U_{x,k}) \leq n\).
	Then let \(W_k = \bigcup\{U_{x,k} : x \in E_{(n)}\}\) and \(G = \bigcap\{W_k : k \in \omega\}\).
	Observe that \(E_{(n)} \subseteq G\) and that \(G\) is a \(G_\delta\) set.

	To see that \(E_{(n)} = G\), let \(x \in G\) and \(\varepsilon > 0\) be arbitrary.
	Let \(k \in \omega\) be so that \(2^{-k} < \varepsilon/2\) and then choose \(y \in E_{(n)}\) to be so that \(x \in U_{y,k}\).
	For \(z \in U_{y,k}\), observe that
	\[d(x,z) \leq d(x,y) + d(y,z) < 2^{-k} + 2^{-k} < \varepsilon\]
	which implies that \(U_{y,k} \subseteq B(x,\varepsilon)\).
	Hence, \(\mathcal N := \{U_{y,k} : y \in E_{(n)}, k \in \omega, x \in U_{y,k}\}\) constitutes a basis at \(x\) with the property that \(\dim(E \cap \partial U) \leq n\) for all \(U \in \mathcal N\).
\end{proof}

\subsection{Subspaces of Metric Spaces}

\begin{definition}
	Suppose \(X\) has metric \(d\).
	\begin{itemize}
		\item
		For \(A \subseteq X\) and \(x\in X\), define \(d(x,A) = \inf\{d(x,y) : y \in A\}\).
		\item
		For any \(E \subseteq X\) and \(A \subseteq E\), define \[\phi_E A = \{ x \in X : d(x,A) \leq d(x,E \setminus A) \}.\]
		\item
		For any \(E \subseteq X\) and \(A \subseteq E\), define \[\gamma_E A = \{ x \in X : d(x,A) < d(x,E \setminus A) \}.\]
	\end{itemize}
\end{definition}
\begin{lemma}
	For any \(A,B \subseteq X\), \(d(x,A \cup B) = \min\{d(x,A),d(x,B)\}\).
\end{lemma}
\begin{proof}
	Since \(A , B \subseteq A \cup B\), we see that \(d(x,A \cup B) \leq \min\{d(x,A),d(x,B)\}\).

	Now, without loss of generality, suppose \(d(x,A \cup B) < d(x,B)\) and let \(\varepsilon > 0\) be so that \[d(x,A \cup B) + \varepsilon < d(x,B).\]
	There exists some \(y \in A \cup B\) so that \(d(x,y) < d(x,A\cup B) + \varepsilon\).
	It must be the case that \(y \in A\).
	Hence, \(d(x,A) \leq d(x,A \cup B)\).
	This finishes the proof.
\end{proof}
\begin{lemma}\label{lem:Decomposition}
	Suppose \(X\) has metric \(d\) and fix \(E \subseteq X\).
	Then, for any \(A,B \subseteq E\), \(\phi_E(A \cup B) = \phi_E(A) \cup \phi_E(B)\).
	Consequently, \(\gamma_E(A \cap B) = \gamma_E(A) \cap \gamma_E(B)\).
\end{lemma}
\begin{proof}
	First, suppose \(x \in \phi_E(A) \cup \phi_E(B)\) and, without loss of generality, assume \(x \in \phi_E(A)\).
	That is, \(d(x,A) \leq d(x,E\setminus A)\).
	Notice that \(d(x,A \cup B) \leq d(x,A)\) and \(d(x,E\setminus A) \leq d(x,E \setminus (A \cup B))\) since \(A \subseteq A \cup B\) and \(X \setminus (A\cup B) \subseteq X \setminus A\).
	Hence,
	\[
		d(x,A \cup B) \leq d(x,A) \leq d(x,E\setminus A) \leq d(x,E \setminus (A \cup B))
	\]
	which establishes that \(x \in \phi_E(A \cup B)\).

	Now, assume that \(x \in \phi_E(A \cup B)\).
	Since \(d(x,A \cup B) = \min\{d(x,A),d(x,B)\}\), without loss of generality, suppose \(d(x,A \cup B) = d(x,A)\).
	As \(x \in \phi_E(A \cup B)\),
	\[
		d(x,A) = d(x,A \cup B) \leq d(x,E \setminus ( A \cup B ))
	\]
	and since, by assumption, \(d(x,A) \leq d(x,B)\), we have that
	\begin{align*}
		d(x,A)
		&\leq \min\{ d(x,E \setminus ( A \cup B )), d(x,B) \}\\
		&= d(x,(E \setminus ( A \cup B )) \cup B)\\
		&= d(x,((E \setminus A) \cap (E \setminus B)) \cup B)\\
		&= d(x,B \cup (E \setminus A))\\
		&\leq d(x, E\setminus A).
	\end{align*}
	That is, \(x \in \phi_E(A)\).


	To see that \(\gamma_E(A \cap B) = \gamma_E(A) \cap \gamma_E(B)\), it suffices to see that \(\gamma_E(A) = X \setminus \phi_E(E \setminus A)\).
	This follows from the observation that \(d(x,A) < d(x,E\setminus A)\) if and only if \(x \not\in \phi_E(E \setminus A)\).
\end{proof}

\begin{theorem} \label{theorem:FinitePairwiseDisjointSubsace}
	Let \(X\) be a metric space and \(E \subseteq X\).
	Suppose \(\mathscr V\) is a family of open subsets relative to \(E\).
	Then there exists \(\Phi : \mathscr V \to \mathscr T_X\) so that \(\Phi(V) \cap E = V\) for all \(V \in \mathscr V\) and
	\[
		\left( \forall \mathscr F \in \left[\mathscr V\right]^{<\omega} \right)\left[ \bigcap \mathscr F = \emptyset \implies \bigcap \Phi\left[\mathscr F\right] = \emptyset \right].
	\]
\end{theorem}
\begin{proof}
	We clam that \(\Phi : \mathscr V \to \mathscr T_X\) defined by \(\Phi(V) = \gamma_E V\) suffices.

	To see that \(\gamma_E V\) is open in \(X\), let \(x \in \gamma_E V\) and note that \(d(x,V) < d(x,E\setminus V)\).
	Let \(\varepsilon > 0\) be so that \(d(x,V) + 3\varepsilon < d(x, E \setminus V)\).
	Then we can find \(y \in V\) so that \(d(x,y) < d(x,V) + \varepsilon\).
	Suppose \(z \in B(x,\varepsilon)\).
	Observe that
	\[
		d(z,V) \leq d(z,y) \leq d(z,x) + d(x,y) < \varepsilon + d(x,V) + \varepsilon = d(x,V) + 2 \varepsilon.
	\]
	On the other hand, for any \(w \in E \setminus V\),
	\[
		d(x,E\setminus V) \leq d(x,w) \leq d(x,z) + d(z,w) \implies d(x,E \setminus V) - d(x,z) \leq d(z,w).
	\]
	\[
		d(x,z) < \varepsilon \implies -\varepsilon < -d(x,z)
	\]
	\[
		d(z,V) < d(x,V) + 2 \varepsilon < d(x,V) + 3\varepsilon - d(x,z) < d(x,E\setminus V) - d(x,z) \leq d(z,w).
	\]
	Since this is true for all \(w \in E \setminus V\), we have that
	\[
		d(z,V) < d(x,V) + 2 \varepsilon \leq d(z,E\setminus V).
	\]
	Hence, \(z \in \gamma_E V\) and we see that \(\gamma_E V\) is open.

	Now we show that \(\gamma_E V \cap E = V\).
	Suppose \(x \in V\) and not that we need only show that \(d(x,E \setminus V) > 0\) since \(d(x,V) = 0\).
	Since \(V\) is relatively open in \(E\), we can find \(U\) open in \(X\) so that \(U \cap E = V\).
	Let \(\varepsilon > 0\) be so that \(B(x,\varepsilon) \subseteq U\).
	For any \(y \in E \setminus V\), \(y \not\in B(x,\varepsilon)\) which means that \(d(x,y) \geq \varepsilon\).
	Since this is true for arbitrary \(y \in E \setminus V\), \(d(x,E \setminus V) \geq \varepsilon\).
	So \(x \in \gamma_E V\).

	Now, suppose \(x \in \gamma_E V \cap E\).
	If \(x \in E \setminus V\), then \(d(x, E\setminus V) = 0\), contradicting \(x \in \gamma_E V\).
	So \(x \in V\).

	Finally, since \(\gamma_E(V \cap W) = \gamma_E(V) \cap \gamma_E(W)\) and \(\gamma_E(\emptyset) = \emptyset\), we see that \(V \cap W = \emptyset \implies \Phi(V) \cap \Phi(W) = \emptyset\).
\end{proof}

%=============================================================================================
%   KURATOWSKI END  ==========================================================================
%=============================================================================================


\newpage





\section{Game stuff}

\textcolor{red}{
As is shown in Theorem \ref{theorem:EnGdelta}, \(E_{(0)}\) is a \(G_\delta\).
However, this isn't of any use for the following reason.}

\textcolor{black!30!blue}{Consider \(\mathbb R\) and \(\mathbb Q\). It should be the case that
\(\mathbb Q_{(0)} = \mathbb R\). So \(\text{ind} \mathbb Q_{(0)} \neq 0\).}


\textcolor{black!30!blue}{In a more tragic direction, consider \(H = [0,1]^\omega\) and \(Q = H \cap \mathbb Q^\omega\).
Since \(Q\) is a countable subset of a separable metric space, it is zero-dimensional.
Moreover, by adding a point to \(Q\), we cannot increase the dimension.
So \(Q_{(0)} = H\).}

\textcolor{red}{However, Engelking's Theorem 4.1.19 states that, for ALL metrizable spaces \(X\),
if \(M \subseteq X\) and \(\text{Ind}(X) \leq n\), there exists a \(G_\delta\) \(M^\star\) so that
\(M \subseteq M^\star\) and \(\text{Ind}(M^\star) \leq n\). Then we just need to tie in the fact
that \(\text{Ind} = \dim\) in the realm of metric spaces.}

For a space \(X\), let \(\mathcal Z_X\) be the collection of zero-dimensional subsets.
Let \(\mathcal Z_X^\ast\) be the collection of zero-dimensional \(G_\delta\) subsets.
We consider the ``point-picking'' game where, in the \(n^{\text{th}}\) inning, One picks \(A_n \in \mathcal Z_X\) and Two responds with an open set \(U_n\) so that \(A_n \subseteq U_n\).
Two is declared the winner if \(\bigcup\{U_n:n\in\omega\}\) is not a cover of \(X\).

{   \color{black!30!blue}
\begin{proposition}
    Let \(\mathcal A\) be a class of subsets of a set \(X\) and, for each \(A \in \mathcal A\), let \(\mathscr F_A \subseteq \{ E \subseteq X : A \subseteq E \}\).
    Suppose further that, for each \(A \in \mathcal A\), there exists a countable subfamily \(\mathscr G_A \subseteq \mathscr F_A\) so that \(A \subseteq \bigcap \mathscr G_A \in \mathcal A\).
    Let \(\mathcal O_{\mathcal A} = \{ \mathscr F_A : A \in \mathcal A \}\) and \(\mathcal C_X(\mathscr F,\mathcal A) = \{ \mathscr U \subseteq \bigcup_{A \in \mathcal A} \mathscr F_A : X = \bigcup\mathscr U\}\).
    Then One has a winning strategy in \(\textsf G_1(\mathcal O_{\mathcal A},\neg \mathcal C_X(\mathscr F,\mathcal A))\)
    if and only if \(X\) is \(\sigma\)-\(\mathcal A\).
\end{proposition}
}

\begin{proposition}\label{gdeltasigma}
    If \(\mathcal A\) has the property that for each \(A\in\mathcal A\) there exists
    a \(G_\delta\) \(A^\star\) with \(A\subseteq A^\star\in\mathcal A\), then
    One has a winning strategy in \(\textsf G_1(\mathscr N[\mathcal A],\neg \mathcal O_X)\)
    if and only if \(X\) is \(\sigma\)-\(\mathcal A\).
\end{proposition}
\begin{proof}
    Of course, if \(X = \bigcup \{A_n:n\in\omega\}\) where \(A_n \in \mathcal A\) for each \(n\in\omega\), then One has a winning strategy.
    So we need only show the other direction.
    
    Suppose \(\sigma\) is winning for ONE;
    let \(\sigma'\) yield corresponding members of \(\mc A\).
    Then \(\sigma'(\tuple{})\in\mc A\), so choose \(U_{\tuple{n}}\) open with
    \(\sigma'(\tuple{n})\subseteq X_{\tuple{}}
    =\bigcap\{U_{\tuple n}:n<\omega\}\in\mc A\).
    Now if \(U_t\) is defined for \(t\leq s\in\omega^{n+1}\), note
    \(\sigma'(\tuple{U_{s\rest 1},\dots,U_{s}})\in\mc A\), so choose
    \(U_{s\concat \tuple{n}}\) open with
    \(\sigma'(\tuple{U_{s\rest 1},\dots,U_{s}})\subseteq X_s =
    \bigcap\{U_{s\concat\tuple n}:n<\omega\}\in\mc A\).
    
    We now show that \(X=\bigcup_{s\in\omega^{<\omega}} X_s\). If not,
    pick \(x\not\in X_s\) for all \(s\in\omega^{<\omega}\).
    We then may define \(f\in\omega^\omega\) such that
    \(x\not\in U_{f\rest n+1}\) for all \(n<\omega\).
    Finally, note that the counterattack \(\tuple{U_{f\rest 1},U_{f\rest 2},\dots}\)
    defeats \(\sigma\), a contradiction.
    
    % Suppose One has a winning strategy \(\sigma\).
    % For each \(A \in \mathcal A\), let \(\mathscr U_A\) be a countable family of
    % open sets so that \(A\subseteq A' = \bigcap \mathscr U_A \in \mathcal A\).
    % Now, let \(T_0 = \{\langle\rangle\}\) and recursively define
    % \[
    %     T_{n+1} = \{ w \concat \langle \sigma(w) , U \rangle : w \in T_n, U \in \mathscr U_{\sigma(w)} \}.
    % \]
    % Then
    % \[
    %     W := \bigcup_{n\in\omega}\bigcup_{w\in T_n} \sigma(w)'
    % \]
    % is a countable union of zero-dimensional \(G_\delta\) sets.
    % We show that \(X = W\).
    
    % Toward a contradiction, suppose \(x \not \in W\).
    % Then \(x \not\in \sigma(\langle\rangle)'\), so let \(A_0=\sigma(\langle\rangle)\).
    % Then we can choose \(U_0 \in \mathscr U_{\sigma(\langle\rangle)'}\) so that
    % \(x\not\in U_0\supseteq A_0\).
    
    % Suppose we have
    % \[
    %     w := \langle A_0, U_0, A_1 , U_1, \ldots , A_n, U_n \rangle \in T_{n+1}
    % \]
    % defined.
    % Now \(x \not\in \sigma(w)'\), so let \(A_{n+1}=\sigma(w)\).
    % We can set \(U_{n+1} \in\mathscr U_{\sigma(w)'}\) to be so that \(x \not\in U_{n+1} \supseteq A_{n+1}\).
    
    % Thus by induction we have constructed a play of the game
    % \(\langle A_0,U_0,A_1,U_1,\dots\rangle\) where \(x\not\in\bigcup_{n<\omega} U_n\),
    % so Two wins, contradicting the fact that \(\sigma\) is a winning strategy for One.
\end{proof}

\begin{corollary}[Corollary to Theorem 27 of CH Closed Discrete Compact Open] \label{sigmaStuff}
    If \(\mathcal Z_X\) consists of \(G_\delta\) sets, One has a winning strategy in \(\textsf G_1(\mathscr N[\mathcal Z_X],\neg \mathcal O_X)\) if and only if \(X = \bigcup \{A_n:n\in\omega\}\) where \(\{A_n :n\in\omega\}\subseteq \mathcal Z_X\).
\end{corollary}





In the realm of metric spaces, all zero-dimensional subsets are contained in zero-dimensional \(G_\delta\) sets, due to Engelking Thm 4.1.19.
Hence, at least in the metric context, all countable-dimensional spaces can be written as the countable union of zero-dimensional \(G_\delta\) sets.

\begin{definition}
    For a topological space \(X\) and collection \(\mathcal A\) of subsets of \(X\),
    let \(\mathcal O[X,\mathcal A]\) be the collection of
    all non-trivial open covers \(\mathscr U\) of \(X\) so that, for any member
    \(A \in\mathcal A\), there exists \(U \in\mathscr U\) so that \(A \subseteq U\).
\end{definition}


Note that \(\mathscr N[\mathcal A]\) is a reflection of \(\mathcal O[X,\mathcal A]\).

\begin{proposition}[Clontz Duality]
    The game \(\textsf{G}_1(\mathcal O[X,\mathcal A] , \mathcal O_X)\) and
    \(\textsf{G}_1(\mathscr N[\mathcal A],\neg\mathcal O_X)\) are dual.
\end{proposition}


To get up to \(\textsf{G}_c(\mathcal O, \mathcal O)\), we may have to allow for countably infinite selections.
The obvious relationship is: given a cover \(\mathscr U\) of \(X\) and a zero-dimensional subset \(E\), there is a refinement \(\mathscr V\) which covers \(E\) that consists of pairwise disjoint open sets.

For any open cover \(\mathscr U\) and zero-dimensional subset \(E\) of \(X\), let \(\mathscr U|_E\) be a refinement \(\mathscr V\) of \(\mathscr U\) consisting of pairwise disjoint open sets that covers \(E\).
Then, if One has a strategy in \(\textsf{G}_c(\mathcal O, \mathcal O)\), we can translate One's play \(\mathscr U\) to \[\mathscr W := \left\{ \bigcup \mathscr U|_E : E \underset{\text{zero-dim}}{\subseteq} X \right\}.\]
This should take winning strategies for One in \(\textsf{G}_c(\mathcal O, \mathcal O)\) to winning strategies for One in \(\textsf{G}_1(\mathcal O_X^{zd},\mathcal O)\) at full and pre-determined information levels, respectively.


{\color{black!30!blue}
\begin{center}
    ?? Suppose \(X\) is metrizable,
    Two has a winning strategy in \(\textsf{G}_c(\mathcal O,\mathcal O)\) implies that \(X\) is strongly paracompact. ??
\end{center}

Let \(\mathscr U\) be an open cover.
Let \(\mathscr U_0\) be an open cover that refines \(\mathscr U\) that consists of sets of radius \(< 1\) so that, for every \(U \in \mathscr U_0\), there exists \(V \in \mathscr U\) so that \(\text{cl}(U) \subseteq V\).
Then Two produces a refinement \(\mathscr V_0\) of \(\mathscr U_0\) consisting of pair-wise disjoint open sets according to their strategy.

Now, for some \(n \in \omega\), suppose we have \(\mathscr U_m\) and \(\mathscr V_m\) defined for all \(m \leq n\).
Set \(W_n = \bigcup_{m \leq n} \bigcup \mathscr V_m\), \(F_n = X \setminus W_n\),
and \(\mathscr W_{n}^\prime = \{ U \in \mathscr U_n : U \cap F_n \neq \emptyset \}\).
We can then find a cover \(\mathscr W_{n}^{\prime\prime}\) of \(F_n\) consisting of open sets in
\(X\) with radius \(< 2^{-n-1}\) that refines \(\mathscr W_n^\prime\) so that, for every
\(U \in \mathscr W_n^{\prime\prime}\), there exists \(V \in \mathscr W_n^\prime\) so that \(\text{cl}(U) \subseteq V\).
Then let \(\mathscr U_{n+1} = \left\{ W_n \right\} \cup \mathscr W_n^{\prime\prime}\).
Two produces a refinement \(\mathscr V^\prime_{n+1}\) of \(\mathscr U_{n+1}\) consisting
of pair-wise disjoint open sets according to their strategy.
Define \(\mathscr V_{n+1} = \{ V \in \mathscr V^\prime_{n+1} : V \cap F_n \neq \emptyset \}\).

This defines the \(\mathscr V_n\) for \(n \in \omega\).
Since Two was playing according to their winning strategy, we claim that
\(\mathscr V^\star = \bigcup_n \mathscr V_n\) is an open cover of \(X\) that
refines \(\mathscr U\).
To see this, since the refining property is immediate, we need only see that \(\bigcup_n \mathscr V_n\) is a cover of \(X\).
Let \(\mathscr V_0^\prime = \mathscr V_0\) and let \(x \in X\) be arbitrary.
Then, let \(n\) be minimal so that there exists \(V \in \mathscr V_n^\prime\) with \(x \in V\).
If \(n = 0\), there is nothing to show.
If \(n > 0\), then \(x \not\in W_{n-1} \implies x \in F_{n-1}\) so let \(V \in \mathscr V_n^{\prime}\) so that
\(x \in V\).
Since \(V \cap F_{n-1} \neq \emptyset\), we see that \(V \in \mathscr V_n\).


Since \(X\) is metrizable, it is paracompact, so we can find a covering refinement \(\mathscr V\) of \(\mathscr V^\star\)
so that \(\mathscr V\) is locally finite.
We wish now to demonstrate that \(\mathscr V\) is actually star-finite.
Toward contradiction, suppose there is some \(V_0 \in \mathscr V\) so that
\(\{ V \in \mathscr V : V \cap V_0 \neq \emptyset \}\) is infinite.
\textcolor{red}{Somehow I want this to build a sequence in \(V_0\) that contradicts something.
Probably not that easy...}
}

{\color{black!50!green}
\emph{Potential counter-example to the claim above:}
Consider the hedgehog space of \(\omega_1\) spinniness.
That is, consider \(X_0 = \{ (\alpha , x) : \alpha < \omega_1, x \in [0,1] \}\) represent the disjoint
union of \(\omega_1\)-many copies of the interval.
Then define \(\simeq\) on \(X_0\) by setting \((\alpha,0) \simeq (\beta,0)\) for
all \(\alpha, \beta < \kappa\) and leaving all other points identified only with themselves.
Then the quotient space \(X = X_0/\simeq\) is the hedgehog space of \(\omega_1\) spinniness.
Alexandroff asserts that this is a metrizable space that is not strongly paracompact.
If \(\mathbf 0\) represents the equivalence class of \((\alpha,0)\),
\(Q = \{ (\alpha, q) : \alpha < \kappa, q \in \mathbb Q \cap (0,1] \}\), and \(Y = X \setminus (Q \cup \{\mathbf 0\})\),
this should represent \(X\) as the finite union of zero-dimensional subsets, at least in the sense of ind.
What about the covering dimension?
Given any cover of \(X\), we first need to define \(f : \omega_1 \to [0,1]\) that determines a neighborhood of
\(\mathbf 0\) refining a particular element of the initial cover.
From there, we can cover the remaining line segments individually.
Such a cover should have order bounded by \(2\) so \(\dim X = 1\).
So it would appear that this is an example of a metrizable space that has the Haver property
that is not strongly paracompact.
}


Assume \(X\) has the strategic Haver property (Two has a winning strategy in the Haver game).
For each \(n \in \omega\), let \(\mathscr U_{\langle n \rangle}\) be a pair-wise disjoint family
of open sets with radii bounded by \(2^{-n}\) produced by Two's winning strategy according to the
initial play of \(2^{-n}\).
Then, let \(X_{\langle \rangle} = \bigcap_{n\in\omega} \bigcup \mathscr U_{\langle n \rangle}\).

Now, suppose we have \(\langle n_1 , \ldots, n_k \rangle\) given.
For each \(n \in \omega\), let \(\mathscr U_{\langle n_1 , \ldots , n_k , n\rangle}\) be a pair-wise
disjoint family of open sets with radii bounded by \(2^{-n}\) produced by Two's winning strategy
according to the sequence of plays \(2^{-n_1}, \ldots , 2^{-n_k} , 2^{-n}\).
Then set \(X_{\langle n_1 , \ldots , n_k \rangle} = \bigcap_{n \in \omega} \bigcup \mathscr U_{\langle n_1 , \ldots , n_k , n\rangle}\).

The goal is to show that \(\dim X_w = 0\) for each \(w \in \omega^{<\omega}\).
To do this, we can resort to the large inductive dimension since \(X\) is metrizable.
So let \(F \subseteq X_w\) be closed and \(U \subseteq X_w\) be open with \(F \subseteq U\).
The goal is to find a clopen set \(V\) so that \(F \subseteq V \subseteq U\).

For \(n \in \omega\), consider
\(\mathscr W_n = \{ W \in \mathscr U_{w \oplus \langle n \rangle} : W \cap F \neq \emptyset\}\).
Notice that \(F \subseteq \bigcup \mathscr W_n\) and that \(\mathscr W_n\) is clopen by the fact that
\(\mathscr U_{w \oplus \langle n \rangle}\) is pair-wise disjoint.

By way of contradiction, suppose that there is no \(n\) so that \(\bigcup \mathscr W_n \subseteq U\).
That is, for every \(n\), \(\bigcup \mathscr W_n \cap X_w \setminus U \neq\emptyset\).

\section{clontz}


\begin{lemma}\label{sigmaMark}
Let \(X\) be \(T_1\).
TWO has mark in \(G_1(\mathcal O(X,\mathcal A),\mathcal O)\) iff
\(X\) is \(\sigma\)-relatively \(\mathcal A\) iff
\(X\) is \(\sigma\)-\(\mathcal A\).
\end{lemma}

\begin{proof}
If \(X\) is \(\sigma\)-(relatively \(\mathcal A\)), choose 
\(R_n\subseteq A_n\in\mathcal A\) such that \(X=\bigcup_{n<\omega}R_n\).
Then \(X=\bigcup_{n<\omega}A_n\), and \(X\) is \(\sigma\)-\(\mathcal A\).

If \(X\) is \(\sigma\)-\(\mathcal A\), let \(X=\bigcup_{n<\omega}A_n\)
for \(A_n\in\mathcal A\). Let \(\sigma(\mathcal U,n)\) contain \(A_n\),
then \(\sigma\) wins.

If \(\sigma\) is a winning Mark, then let
\[ R_n = \bigcap_{\mathcal U\in\mathcal O(X,\mathcal A)}\sigma(\mathcal U,n)\]

Then note that \(X=\bigcup_{n<\omega}R_n\); if not, pick \(x\not\in R_n\) for
all \(n<\omega\). Then pick \(\mathcal U_n\in\mathcal O(X,\mathcal A)\) with
\(x\not\in \sigma(\mathcal U_n,n)\) for all \(n<\omega\). Then \(\mathcal U_n\)
defines a play by ONE that beats \(\sigma\), contradiction.

Finally, note that \(R_n\subseteq A\) for some \(A\in\mathcal A\). If not,
then pick \(x_A\in R_n\setminus A\) for each \(A\in\mathcal A\). Then
\(\mathcal U=\{X\setminus\{x_A\}:A\in\mathcal A\}\in\mathcal U(X,\mathcal A)\).
But then pick \(A\) where \(\sigma(\mathcal U,n)=X\setminus\{x_A\}\). Then
\(R_n\not\subseteq\sigma(\mathcal U,n)\), contradiction.
\end{proof}

\begin{corollary}
Let \(X\) be \(T_1\). Then TWO has a winning Markov strategy for
\(G_1(\mathcal O^{zd},\mathcal O)\) iff ONE has a winning predetermined strategy
for \(G_1(\mathcal N[\mathcal Z],\neg\mathcal O)\) if and only if \(X\) is
countable-dimensional.
\end{corollary}

{\color{purple}
\begin{proposition}
If \(TWO\markwin G_c(\mathcal O,\mathcal O)\), then
\(X\) is \(\sigma\)-\(\dim\)-\(0\).
\end{proposition}
\begin{proof}
Let \(\sigma\) be a winning Markov strategy for TWO.
Let \(X_n=\bigcap_{\mathcal U\in\mathcal O}\bigcup\sigma(\mathcal U,n)\). Let
\(\mathcal U\) cover \(X_n\), then \(\sigma(\mathcal U,n)\) is a pairwise disjoint refinement
of \(\mathcal U\) and covers \(X_n\). Therefore \(\dim X_n=0\).

Then consider \(x\in X\). If \(x\not\in X_n\) for all \(n<\omega\), choose
\(\mathcal U_n\in\mathcal O\) with \(x\not\in\bigcup\sigma(\mathcal U_n,n)\).
Then \(\mathcal U_n\) is a successful counterattack to the winning strategy \(\sigma\),
a contradiction. Therefore \(x\in X_n\) for some \(n<\omega\), and
\(X=\bigcup_{n<\omega} X_n\).
\end{proof}
}

{\color{purple}
\begin{theorem}
The following are equivalent for a strongly paracompact (e.g. separable) metric space
\(\tuple{X,d}\).
\begin{enumerate}
    \item \(X\) is \(\sigma\)-zero-dimensional.
    \item \(TWO\win H(X,d)\)
    \item \(TWO\markwin H(X,d)\)
    \item \(TWO\win G_c(\mathcal O,\mathcal O)\)
    \item \(TWO\markwin G_c(\mathcal O,\mathcal O)\)
    \item \(TWO\win G_c(\mathcal O_{diam},\mathcal O)\)
    \item \(TWO\markwin G_c(\mathcal O_{diam},\mathcal O)\)
    \item \(TWO\win G_1(\mathcal O_Z,\mathcal O)\)
    \item \(TWO\markwin G_1(\mathcal O_Z,\mathcal O)\)
    \item \(ONE\win G_1(\mathcal N_Z,\neg\mathcal O)\)
    \item \(ONE\prewin G_1(\mathcal N_Z,\neg\mathcal O)\)
\end{enumerate}
\end{theorem}
\begin{proof}
The equivalence of (1/2/4/6) is from Count Dim, A Game, etc..
Then to see (1) implies (5), let \(X=\bigcup_{n<\omega}Z_n\)
with \(Z_n\) zero-dimensional. Since \(\dim Z_n=0\), let
\(\sigma(\mathcal U,n)\) be a pairwise disjoint open refinement
of \(\mathcal U\) that covers \(Z_n\); it follows that
\(\sigma\) is a winning Markov strategy for TWO.
Then (5) implies (7) implies (3) implies (2) are all direct,
yielding the equivalence of (1-7).

To see (1) implies (11), let \(X=\bigcup_{n<\omega}Z_n\)
with \(Z_n\) zero-dimensional. Then if \(\sigma(n)\)
is the collection of open sets containing \(Z_n\),
it follows that \(\sigma\) is a winning predetermined
strategy for ONE. Then (11) implies (10) directly,
and (10) is equivalent to (1) by Theorems \ref{gdeltasigma}
and \ref{metgdeltazd}.

Finally (8/9) are equivalent to the rest via duality with
(10/11).
\end{proof}

(note: \(H(X,d)\) doesn't make sense without metric,
although could swap the metric with a uniformity I guess.
When you drop metrizable then the \(G_c\) games might
work with \(\dim X=0\) and Markov strats, and
the \(G_1\) games might work with \(\mathrm{ind} X=0\)
and Markov strats. Would be nice if we had a non-metrizable
counterexample where
\(ONE\win G_1(\mathcal N_Z,\neg\mathcal O)\) but
is not countable-dimensional.


CLONTZ TODO: wire up markov strategies with \(<\) sepMet.

CLONTZ TODO: maybe consider Haver game with entourages
}


\newpage


\begin{example}
Let \(N=\mathbb R\times[0,\infty)\)
have Niemytzki's tangent disc topology.
For \(B\subseteq\mathbb R\), let
\(N(B)=N\setminus((\mathbb R\setminus B)\times\{0\})\)
be the bubble space of \(B\).

Note that since \(\mathbb R\times(0,\infty)\)
is an open copy of the Euclidean plane, each point here
has a basis of open sets with boundaries
of inductive dimension \(1\).

Consider the point \(\tuple{z,0}\). By definition it has
the basis of open sets
\[
B_a(z)=
\{\tuple{x,y}:(x-z)^2+(y-a)^2<a^2\}\cup\{\tuple{z,0}\}
\]
where each boundary is given by
\[
\partial B_a(z)=
\{\tuple{x,y}:(x-z)^2+(y-a)^2=a^2\}\setminus\{\tuple{z,0}\}
.\]
As \(\partial B_a(z)\) is homeomorphic to the Euclidean
line, it follows that each \(\partial B_a(z)\) has inductive
dimension \(1\).

We have thus shown that \(\ind N(B)\leq 2\) for any
\(B\subseteq\mathbb R\), and therefore
\(TWO\markwin G_1(\mc O[Z_{\ind}],\mc O)\) for \(N(B)\).
Likewise \(\dim N(B)\leq 2\) as it is the union of \(0\)-\(\dim\)
\(x\)-axis and the \(2\)-\(\dim\) upper plane.
However, \(N(B)\) is not screenable if \(B\) is uncountable,
and therefore ONE has a winning strategy in \(G_c(\mc O,\mc O)\).
To see this, consider the open cover
\(\mc U=\{\mathbb R\times(0,\infty)\}\cup\{B_1(z):z\in\mathbb R\}\).
For any pairwise disjoint refinement of this cover,
only countably-many points \(\tuple{z,0}\) can be covered, as
any open subset of \(B_1(z)\) containing \(\tuple{z,0}\)
must contain a point in the countable set \(\mathbb Q^2\).
Thus \(\mc U\) lacks a \(\sigma\)-pairwise-disjoint refinement
covering \(N(B)\).

% According to the pi-base, the Niemytzki plane is not countably paracompact
% so the covering dimension is not finite. (SC: why?)
If the open cover
\(\mc U=\{\mathbb R\times(0,\infty)\}\cup\{B_1(z):z\in\mathbb R\}\)
has a pairwise-disjoint open refinement covering \(Y\), then by the 
above argument, \(Y\) contains only countably-many members of \(B\times\{0\}\).
Thus \(N(B)\) is not \(\sigma\)-\(\dim_X\)-\(0\) for \(B\) uncountable.

Suppose that if \(B\) is a \(Q\)-set, that is,
an uncountable set such that every subset of \(B\)
is \(F_\sigma\) relative to \(B\). Such sets exist assuming
\(MA+\neg CH\), in fact, every \(\aleph_1\) subset of \(\mathbb R\)
is a \(Q\)-set [cite Fleissner/Miller - On Q sets].
Furthermore, it is known that \(N(B)\) is normal when \(B\) is a \(Q\)-set
[cite Bing - Metrization of topological spaces].

Therefore \(N(B)\) with \(|B|=\aleph_1\) is an example of a
\(T_{3.5}\) (consistently \(T_4\)) space with finite inductive and
covering dimension, but TWO does not have a wininng strategy in
\(G_c(\mc O,\mc O)\) and it 
is not the countable union of \(\dim_X\)-\(0\) subsets.
\end{example}

Can we get a normal but non-metrizable example? (SC: yes consistently, see above)

Suppose Two has a Markov strategy \(\tau\) in the entourage Haver game.
Let \(X_n = \bigcap \{ \bigcup \tau(\mathscr U, n) : \mathscr U \in \mathcal O_X \}\).
Fix a point \(x \in X_n\) and an open entourage \(U_0\), and let \(U\) be a symmetric entourage so that \(U \circ U \subseteq U_0\).
Since \(\mathscr U := \{ U[y] : y \in X \} \in \mathcal O_X\), \(\tau(\mathscr U,n)\) is
a collection of pair-wise disjoint open sets that refines \(\mathscr U\).
Let \(V \in \tau(\mathscr U, n)\) that contains \(x\) and notice that \(x \in V \subseteq U[y]\) for some \(y \in X\).
For \(z \in V\), this means that \((z,y) \in U\) and, since \((x,y) \in U\) and \(U\) is symmetric, we see that \((z,x) \in U_0\).
So \(V \subseteq U_0[x]\).
Notice that \(W := \bigcup \{ G \in \tau(\mathscr U , n) : G \neq V \}\) is open and that \(V \cap W = \emptyset\).
So \(\overline{V} \cap W = \emptyset\) and we see that \(X_n \cap V = X_n \cap \overline{V}\).

\newpage

\section{Zero-Dimension and Subsets/Subspaces}

A space \(X\) is \(0\)-\(\dim\) if for every open cover of \(X\),
there exists a pairwise disjoint open refinement covering \(X\).

A subset \(Y\subseteq X\) is \(0\)-\(\dim_X\) if for every cover of \(Y\)
by sets open in \(X\),
there exists a pairwise disjoint open refinement covering \(Y\).

\begin{example}
Let \(B\subseteq\mathbb R\) have cardinality \(\aleph_1\).
The discrete subset \(Y=B\times\{0\}\) of the bubble space \(X=N(B)\) is an example
of a subset of a \(T_{3.5}\) (consistently \(T_4\)) space which is
\(0\)-\(\dim\), but not \(\sigma\)-\(0\)-\(\dim_X\).
\end{example}

\begin{proposition}
For every \(Y\subseteq X\),
if \(Y\) is \(0\)-\(\dim_X\), then \(Y\) is \(0\)-\(\dim\).
\end{proposition}
\begin{proof}
Assume \(Y\) is \(0\)-\(\dim_X\). Let \(\mc U\) be a cover of \(Y\) by
open subsets of \(Y\). Let \(\mc U'\) be a collection of open subsets of
\(X\) such that for each \(U\in \mc U\) there exists \(U'\in\mc U'\)
such that \(U=U'\cap Y\). Let \(\mc V'\) be a pairwise-disjoint open refinement
of \(\mc U'\) covering \(Y\). Let \(\mc V=\{V'\cap Y:V'\in\mc V'\}\).
It follows that \(\mc V\) is a pairwise disjoint refinement of \(\mc U\)
of sets open in \(Y\) that covers \(Y\), so \(Y\) is \(0\)-\(\dim\).
\end{proof}
\begin{theorem}
Let \(X\) be metrizable. Then for every \(Y\subseteq X\),
\(Y\) is \(0\)-\(\dim_X\) if and only if \(Y\) is \(0\)-\(\dim\).
\end{theorem}
\begin{proof}
Assume \(Y\) is \(0\)-\(\dim\). Let \(\mc U=\{U_\alpha:\alpha<\kappa\}\)
be a cover of \(Y\) by open
subsets of \(X\). Then \(\mc U'=\{U'_\alpha:\alpha<\kappa\}\)
where \(U'_\alpha=U_\alpha\cap Y\) for each \(\alpha<\kappa\) is a cover of \(Y\)
by open subsets of \(Y\). Let
\(\mc V'=\{V'_{\alpha,\beta}:\alpha<\kappa,\beta<\lambda_\alpha\}\)
where \(V'_{\alpha,\beta}\subseteq U'_\alpha\)
be a pairwise-disjoint refinement of \(\mc U'\)
by sets open in \(Y\) covering \(Y\). By [Kuratowski II.XI.21.2] and
the metrizability of \(X\),
there exists a pairwise disjoint collection
\(\mc V=\{V_{\alpha,\beta}:\alpha<\kappa,\beta<\lambda_\alpha\}\) of sets open
in \(X\) such that \(V'_{\alpha,\beta}=V_{\alpha,\beta}\cap Y\).
Let \(W_{\alpha,\beta}=V_{\alpha,\beta}\cap U_\alpha\), so
\(\mc W=\{W_{\alpha,\beta}:\alpha<\kappa,\beta<\lambda_\alpha\}\) is a
pairwise disjoint refinement of \(\mc U\) by sets open in \(X\).
Let \(y\in Y\), and choose \(\alpha<\kappa,\beta<\lambda_\alpha\) such that
\(y\in V'_{\alpha,\beta}\). Then both
\(y\in V'_{\alpha,\beta}\subseteq U_\alpha'\subseteq U_\alpha\)
and \(y\in V'_{\alpha,\beta}\subseteq V_{\alpha,\beta}\), so \(y\in W_{\alpha,\beta}\).
Thus \(\mc W\) covers \(Y\), and \(Y\) is \(0\)-\(\dim_X\).
\end{proof}

\begin{theorem}
\(TWO\markwin G_c(\mathcal O,\mathcal O)\) if and only if
\(X\) is \(\sigma\)-\(\dim_X\)-\(0\).
\end{theorem}
\begin{proof}
Let \(\tau\) be a winning Markov strategy for TWO.
Let \(X_n=\bigcap_{\mathcal U\in\mathcal O}\bigcup\tau(\mathcal U,n)\). Let
\(\mathcal U\) cover \(X\), then \(\tau(\mathcal U,n)\) is a pairwise disjoint refinement
of \(\mathcal U\) and covers \(X_n\). Therefore \(X_n\) is \(0\)-\(\dim_X\).

Then consider \(x\in X\). If \(x\not\in X_n\) for all \(n<\omega\), choose
\(\mathcal U_n\in\mathcal O\) with \(x\not\in\bigcup\tau(\mathcal U_n,n)\).
Then \(\mathcal U_n\) is a successful counterattack to the winning strategy \(\tau\),
a contradiction. Therefore \(x\in X_n\) for some \(n<\omega\), and
\(X=\bigcup_{n<\omega} X_n\). Thus \(X\) is \(\sigma\)-\(0\)-\(\dim_X\).

Now assume \(X=\bigcup_{n<\omega}X_n\) with \(X_n\) \(\dim_X\)-\(0\).
Let \(\tau(\mc U,n)\) be a pairwise disjoint open refinement of \(\mc U\)
covering \(X_n\).
It follows that \(\tau\) is a winning Markov strategy for TWO.
\end{proof}

\begin{claim}
Suppose every \(\dim_X\)-\(0\) subset of \(X\) is contained in a
\(G_\delta\) and \(\dim_X\)-\(0\) set. Then
\(TWO\win G_c(\mc O,\mc O)\) if and only if
\(X\) is \(\sigma\)-\(\dim_X\)-\(0\).
\end{claim}

\begin{proof}
Let \(\tau\) be a winning strategy for TWO in \(G_c(\mc O,\mc O)\).
Then \(X_{\tuple{}}=\bigcap_{\mc U\in\mc O}\bigcup\tau(\tuple{\mc U})\)
is \(\dim_X\)-\(0\) and contained in a \(\dim_X\)-\(0\)
\(X'_{\tuple{}}=\bigcap_{n<\omega}U_{\tuple{n}}\) with \(U_{\tuple{n}}\)
open and \(U_{\tuple{n}}\supseteq U_{\tuple{n+1}}\).
So let \(\tau'(\tuple{\mc U})\) be a pairwise-disjoint open refinement
of \(\mc U\) covering \(X'_{\tuple{}}\) by subsets of \(U_{\tuple{0}}\)...
\end{proof}

\begin{claim}
Let \(\mc A=\{A_{\mc U}:\mc U\in\mc O\}\) where
\(A_{\mc U}=\{\mc V:\mc V\text{ is pwdor of }\mc U\}\).
Let \(\mc R=\{R_Z:\dim_X Z=0\}\) where
\(R_Z=\{\mc V:\mc V\text{ is pwdoc of }Z\}\).
Let \(\hat{\mc O}=\{\hat{\mc U}:\bigcup\hat{\mc U}\in\mc O\}\).

Then
\(G_c(\mc O,\mc O)\) is equivalent to
\(G_1(\mc A,\hat{\mc O})\) is dual to
\(G_1(\mc R,\neg\hat{\mc O})\) is equivalent to
\(G_1(\mc N[Z],\neg{\mc O})\).
\end{claim}

\begin{proof}
To see that
\(G_c(\mc O,\mc O)\) is equivalent to
\(G_1(\mc A,\hat{\mc O})\), note that for each \(\mc U\in\mc O\)
there is a unique corresponding \(A\in\mc A\), and vice versa.
Then, the possible moves of TWO from these corresponding moves
are identical for each,
and the winning condition for each game given these choices
are identical.

To see that
\(G_1(\mc A,\hat{\mc O})\) is dual to
\(G_1(\mc R,\neg\hat{\mc O})\), we will
show \(\mc R\) is a reflection of \(\mc A\).
Therefore we need
for each \(A_{\mc U}\in\mc A\) some
\(f_{\mc U}:\mc R\to\bigcup\mc R\) with \(f_{\mc U}(R_Z)\in R_Z\),
\(ran f_{\mc U}\subseteq A_{\mc U}\), and \(ran f_{\mc U}\in\mc A\).

Let's assume the answer to
https://mathoverflow.net/questions/402238
is yes.
Enumerate \(A_{\mc U}=\{\mc V_{\alpha}:\alpha<\kappa\}\)
and note that each \(Z_\alpha\) constructed in that question
is \(\dim_X\)-\(0\).
For \(R_Z\in\mc R\), suppose \(Z=Z_\alpha\) for some
\(\alpha<\kappa\); then let \(f_{\mc U}(R_Z)=\mc V_\alpha\),
so \(ran f_{\mc U}\supseteq A_{\mc U}\).
Otherwise, let \(f_{\mc U}(R_Z)\in A_{\mc U}\)
be the pairwise-disjoint
open refinement of \(\mc U\) covering \(Z\) witnessed by \(\dim_X Z=0\),
so \(ran f_{\mc U}\subseteq A_{\mc U}\). Therefore 
\(ran f_{\mc U}=A_{\mc U}\in\mc A\), and \(\mc R\) is a
reflection, demonstrating duality.

To see that
\(G_1(\mc R,\neg\hat{\mc O})\) is equivalent to
\(G_1(\mc N[Z],\neg{\mc O})\), note that for each \(\mc U\in\mc N[Z]\)
there is a unique corresponding \(R\in\mc R\), and vice versa.
Then, the possible moves of TWO from these corresponding moves
are almost identical for each (modulo the different choices of
pairwise disjoint open covers of \(Z\) that union to the same set),
and the winning condition for each game given these choices
are identical.
\end{proof}



If Two can win, Two can win where, in each inning, the union of their play is dense.

For \(\mathbb Q\), every open set is countable.
There are \(\mathfrak c\)-many countable subsets, all of which are relatively zero-dim.
(Each of these is of cardinality \(<\) the cardinality of any open set.)
There are \(\mathfrak c\)-many collections of pairwise disjoint open sets.

We need the collection of all relatively zero-dim subspaces to be cardinality \(\geq\) the cardinality of collections of pairwise disjoint open sets.
\(\mathfrak Z\) all relatively zero-dim subspaces. We want some \(\mathfrak Z' \subseteq \mathfrak Z\) so that the cardinality condition
above is satisfied.
We also need every open set to contain \(|\mathfrak Z'|\)-many relatively zero-dim of \(\mathfrak Z'\).

\newpage 


\section{ABANDONED: Equivalence of \texorpdfstring{\(G_c(\mc O,\mc O)\)}{G\_c(O,O)} and
\texorpdfstring{\(G_1(\mc O_{0\dim_X},\mc O)\)}{G\_1(O[Z\_(0dim\_X)],O)}}

Conjecture \ref{conjEq} would be quickly verified by
a proof of the following stronger conjecture.

\begin{conjecture}
The games \(G_c(\mc O,\mc O)\) and
\(G_1(\mc O_{0\dim_X},\mc O)\) are equivalent.
\end{conjecture}

While the validity of this general claim remains an open question,
we are able to verify the following special case.

\begin{theorem}
Suppose each open subset of \(X\) contains at least as
many zero-dim\(_X\) subsets as there are collections of
pairwise-disjoint open subsets of \(X\). Then
the games \(G_c(\mc O,\mc O)\) and
\(G_1(\mc O_{0\dim_X},\mc O)\) are equivalent.
\end{theorem}

\begin{proof}
Let \(\mc A=\{A_{\mc U}:\mc U\in\mc O\}\),
where \(A_{\mc U}\) collects all of the pairwise-disjoint
open refinements of \(\mc U\).
In addition,
let \(\mc R=\{R_Z:Z\text{ is } 0\dim_X\}\), where
\(R_Z\) collects all pairwise-disjoint collections of open
sets where \(Z\subseteq\bigcup R_Z\).
Finally,
let \(\hat{\mc O}=\{C:\bigcup C\in\mc O\}\).

Then the claimed equivalence will be established by way of
the auxiliary
games \(G_1(\mc A,\hat{\mc O})\),
\(G_1(\mc R,\neg\hat{\mc O})\), and
\(G_1(\mc N_{0\dim_X},\mc O)\).
In particular, we will show that
\begin{itemize}
    \item 
the games \(G_c(\mc O,\mc O)\) and
\(G_1(\mc A,\hat{\mc O})\) are equivalent,
    \item
the games \(G_1(\mc A,\hat{\mc O})\) and
\(G_1(\mc R,\neg\hat{\mc O})\) are dual,
    \item
the games \(G_1(\mc R,\neg\hat{\mc O})\) and
\(G_1(\mc N_{0\dim_X},\neg\mc O)\) are equivalent, and
    \item
the games \(G_1(\mc N_{0\dim_X},\neg\mc O)\) and
\(G_1(\mc O_{0\dim_X},\mc O)\) are dual.
\end{itemize}

To see that
\(G_c(\mc O,\mc O)\) is equivalent to
\(G_1(\mc A,\hat{\mc O})\), for any move by ONE in
either game, there is a corresponding move by ONE in the other
game that presents TWO with the same options. Since the winning
conditions for both games are identical and based only on
the choices made by TWO, the result follows.

To see that
\(G_1(\mc A,\hat{\mc O})\) is dual to
\(G_1(\mc R,\neg\hat{\mc O})\), we will
show \(\mc R\) is a reflection of \(\mc A\).
Therefore we need
for each \(A_{\mc U}\in\mc A\) some
\(f_{\mc U}:\mc R\to\bigcup\mc R\) with \(f_{\mc U}(R_Z)\in R_Z\),
\(\ran f_{\mc U}\subseteq A_{\mc U}\), and \(\ran f_{\mc U}\in\mc A\).
In fact, we will define \(f_{\mc U}\) where
\(\ran f_{\mc U}=A_{\mc U}\in\mc A\).

Enumerate \(A_{\mc U}=\{\mc V_{\alpha}:\alpha<\kappa\}\).
We will define zero-dim\(_X\) sets \(Z_\alpha\) distinct for
each \(\alpha<\kappa\).
Assuming \(Z_\beta\) has been defined for \(\beta<\alpha\),
consider the open set \(V_\alpha=\bigcup V_\alpha\).
Every open set contains at least \(\kappa\)-many zero-dim\(_X\)
subsets, so we may choose a zero-dim\(_X\) set
\(Z_\alpha\subseteq V_\alpha\) distinct from \(Z_\beta\)
for all \(\beta<\alpha<\kappa\).
Then for each \(R_Z\in\mc R\), suppose \(Z=Z_\alpha\) for some
\(\alpha<\kappa\); in this case, let
\(f_{\mc U}(R_Z)=\mc V_\alpha\in R_Z\cap A_{\mc U}\).
Otherwise, let \(f_{\mc U}(R_Z)\in R_Z\cap A_{\mc U}\)
be any pairwise-disjoint
open refinement of \(\mc U\) covering \(Z\) guaranteed by \(\dim_X Z=0\),
Since each \(\mc V_\alpha\) is mapped to, we have established
that \(\mc R\) is a reflection of \(\mc A\), and therefore the games
are dual.

To see that
\(G_1(\mc R,\neg\hat{\mc O})\) is equivalent to
\(G_1(\mc N_{0\dim_X},\neg{\mc O})\), consider a move \(R_Z\in\mc R\)
by ONE in the first game, to which TWO may respond with some pairwise
disjoint open collection \(\mc V\in R_Z\). The union of this pairwise
disjoint collection is an open set \(U\) that contains \(Z\), and
\(\{U\}\) is a pairwise disjoint collection that covers \(Z\).
Replacing the original choice with \(\{U\}\in\ R_Z\) has no effect on
the outcome of the game, so we may assume TWO always chooses sets
in this form. Likewise, for every move \(N_Z\) by ONE
in the second game, player two must choose some open set \(U\) containing
\(Z\), corresponding to the pairwise disjoint open collection \(\{U\}\in R_Z\).
Since the moves \(\tuple{\{U_0\},\{U_1\},\dots}\) by TWO in
\(G_1(\mc R,\neg\hat{\mc O})\) win the game if and only if
the moves \(\tuple{U_0,U_1,\dots}\) by TWO in
\(G_1(\mc N_{0\dim_X},\neg{\mc O})\) win that game, the result follows.

Finally, the duality of 
the games \(G_1(\mc N_{0\dim_X},\neg\mc O)\) and
\(G_1(\mc O_{0\dim_X},\mc O)\) was noted in Proposition
\ref{dualGames}.
\end{proof}


{   \color{black!50!blue!60}
[CHRIS DOUBLE CHECK]
\(\mathcal A = \{ A_{\mathscr U} : \mathscr U \in \mathcal O \}\) where \(A_{\mathscr U}\)
is the set of all pairwise disjoint refinements of \(\mathscr U\).
\(\mathcal R = \{ R_Z : Z\text{ is } 0\dim_X \}\) where \(R_Z\) consists of all collections \(\mathscr V\)
of pairwise disjoint open sets so that \(Z \subseteq \bigcup \mathscr V\).
\(\hat{\mathcal O} = \{ C \subseteq \wp(\wp(X)) : \bigcup C \in \mathcal O \}\).

For the equivalence of \(\mathsf G_c(\mathcal O,\mathcal O)\) and \(\mathsf G_1(\mathcal A, \hat{\mathcal O})\),
we consider how to translate between the two games.
For any play \(\mathscr U\) of One in \(\mathsf G_c(\mathcal O,\mathcal O)\), One can play \(A_{\mathscr U}\)
in \(\mathsf G_1(\mathcal A, \hat{\mathcal O})\).
In \(\textsf G_c(\mathcal O,\mathcal O)\), if Two responds with a family \(\mathscr V\) consisting
of pairwise disjoint open sets that refines \(\mathscr U\), then \(\mathscr V \in A_{\mathscr U}\).
Also, clearly, if Two responds with \(\mathscr V \in A_{\mathscr U}\), then \(\mathscr V\)
is a pairwise disjoint refinement of \(\mathscr U\) consisting of pairwise disjoint open sets.

So we now look at the winning condition.
In \(\mathsf G_c(\mathcal O,\mathcal O)\), Two wins iff their sequence of plays
\(\langle\mathscr V_n : n \in \omega\rangle\) satisfies \(\bigcup_{n\in\omega} \bigcup \mathscr V_n = X\).
In \(\mathsf G_1(\mathcal A, \hat{\mathcal O})\), Two wins iff their sequence of plays
\(\langle\mathscr V_n : n \in \omega\rangle\) satisfies \(\bigcup_{n\in\omega} \mathscr V_n \in \mathcal O\).
Since the winning conditions are the same and the translation between games is coherent,
the equivalence is obtained.

For the duality of \(\mathsf G_1(\mathcal A, \hat{\mathcal O})\) and \(\mathsf G_1(\mathcal R, \neg\hat{\mathcal O})\),
we check that \(\mathcal R\) is a reflection of \(\mathcal A\).
For \(\mathscr U \in \mathcal O\), we first enumerate \(A_{\mathscr U} = \{ \mathcal V_\alpha : \alpha < \kappa \}\).
We now define a family of zero-dim\(_X\) subspaces according to each \(\alpha < \kappa\) as follows:
Assume that, for \(\alpha < \kappa\), \(\{ Z_\beta : \beta < \alpha\}\) have been defined to be pairwise distinct
zero-dim\(_X\) subspaces so that \(Z_\beta \subseteq \bigcup \mathcal V_\beta\) for each \(\beta < \alpha\).
Now, by hypothesis, \(\bigcup\mathcal V_\alpha\) contains \(\kappa\)-many zero-dim\(_X\) subsets.
So then there must be some \(Z_\alpha \not\in \{ Z_\beta : \beta < \alpha \}\) with
\(Z_\alpha \subseteq \bigcup \mathcal V_\alpha\).
Now we define \(f_{\mathscr U} : \mathcal R \to \bigcup \mathcal R\) as follows:
For \(R_{Z_\alpha}\), \(\alpha < \kappa\), we set
\(f_{\mathscr U}(R_{Z_\alpha}) = \mathcal V_\alpha \in R_{Z_\alpha} \cap A_{\mathscr U}\).
If \(Z \not\in \{ Z_\alpha : \alpha < \kappa \}\), then define \(f_{\mathscr U}(Z) \in R_Z \cap A_{\mathscr U}\),
any pairwise disjoint family of open sets covering \(Z\) that refines \(\mathscr U\).

Since \(f_{\mathscr U}(Z_\alpha) = \mathcal V_\alpha\) for each \(\alpha < \kappa\), we see that
\(\mathrm{ran}(f_{\mathscr U}) = A_{\mathscr U}\).

\textcolor{red}{Okay, but what about for other \(f \in \mathbf C(\mathcal R)\)?
The point is to show that \(\{ \mathrm{ran}(f) : f \in \mathbf C(\mathcal R)\}\) is a selection basis for \(\mathcal A\).
To establish that, we first need to show that \(\{ \mathrm{ran}(f) : f \in \mathbf C(\mathcal R)\} \subseteq \mathcal A\).}
}

\begin{lemma}
Let \(X\) be metrizable and satisfy the countable
chain condition.
Then each open subset of \(X\) contains at least as
many zero-dim\(_X\) subsets as there are collections of
pairwise-disjoint open subsets of \(X\).
\end{lemma}

\begin{proof}
TODO (actually fix the lemma - a countable discrete space is
a counter-example)


(ISOLATED POINTS?)
The set of isolated points is open.
If we can win on \(X\), then we should be able to win on a closed subspace of \(X\)
by extending open covers in the natural way...

(COMMENTARY)
Suppose \(X\) is a ccc metrizable space with no isolated points.
Every open set is at least countable and thus contains at least \(\mathfrak c\) many zero-dim subspaces.
Let \(w(X)\) be the weight of \(X\) and notice that there are at most \(2^{w(X)}\) distinct open sets.
Then, by the ccc property, there are at most \((2^{w(X)})^\omega = 2^{w(X)}\) families of pairwise disjoint open sets.
\textcolor{red}{However, as it turns out, ccc metrizable spaces are separable so \(w(X) = \omega\).}

It seems that the required condition here is \(2^{w(X)} \leq d(x)^\omega\)
unless we start throwing in uncountable zero-dimensional subspaces.


(SKETCH)
The argument is effectively as follows.
Assume \(\kappa\) is regular.
Enumerate the distinguished family \(\mathcal Z_0 = \{ Z_\alpha : \alpha < \kappa\}\) of zero-dimensional subspaces
and enumerate \(\mathcal{PD} = \{ \mathcal V_\alpha : \alpha < \kappa \}\).
For \(\mathcal V_0\), let \(\eta(0) < \kappa\) be so that \(Z_{\eta(0)} \subseteq \bigcup \mathcal V_0\).

Suppose we have \(\mathcal V_\beta\) and \(\eta(\beta)\) defined for all \(\beta < \alpha < \kappa\) so that \(\eta(\gamma) < \eta(\beta)\) for any \(\gamma < \beta < \alpha\).
Then \(\sup\{ \eta(\beta) : \beta < \alpha \} < \kappa\) since \(\kappa\) is regular.
For \(\mathcal V_\alpha\), let \(\eta(\alpha) \in (\sup \{ \eta(\beta) : \beta < \alpha \}, \kappa)\)
be so that \(Z_{\eta(\alpha)} \subseteq \bigcup \mathcal V_\alpha\).
This is possible since every open set contains \(\kappa\)-many sets from \(\mathcal Z_0\).


\end{proof}

\begin{corollary}
Let \(X\) be metrizable and satisfy the countable
chain condition. Then
the games \(G_c(\mc O,\mc O)\) and
\(G_1(\mc O_{0\dim_X},\mc O)\) are equivalent.
\end{corollary}

